"Did They F***ing Consent to That?": Safer Digital Intimacy via Proactive Protection Against Image-Based Sexual Abuse

As many as 8 in 10 adults share intimate content such as nude or lewd images. Sharing such content has significant benefits for relationship intimacy and body image, and can offer employment. However, stigmatizing attitudes and a lack of technological mitigations put those sharing such content at risk of sexual violence. An estimated 1 in 3 people have been subjected to image-based sexual abuse (IBSA), a spectrum of violence that includes the nonconsensual distribution or threat of distribution of consensually-created intimate content (also called NDII). In this work, we conducted a rigorous empirical interview study of 52 European creators of intimate content to examine the threats they face and how they defend against them, situated in the context of their different use cases for intimate content sharing and their choice of technologies for storing and sharing such content. Synthesizing our results with the limited body of prior work on technological prevention of NDII, we offer concrete next steps for both platforms and security & privacy researchers to work toward safer intimate content sharing through proactive protection. Content Warning: This work discusses sexual violence, specifically, the harms of image-based sexual abuse (particularly in Sections 2 and 6).

==> miscell.tex <==
"But now I just only share these images with like, a person of  confidence. I am really, really confident in this person. When I was younger, I used to be a bit more careless and send it to other people who I was not really confident with them. So I.. Yeah, so the safety was important then. Now, yeah, I trust my partners. So it's, it's fine, if he screens them it's very, it's really fine."P30


I never put it anywhere else, because I don't have the knowledge of where to put it, basically. And now I am just doing it a bit precariously just using what I have, and not really giving much importance of where or the privacy or any other thing. It's something I want to work on, but it's just what I have now. P9

when work is shared without your consent, when you send it to a client, and that's been shared onto another platform without your consent. There's no question that when it gets to that stage, there's no control over it. So I think there's the conversation that comes up with online sex workers is, is that sort of like, like, where's the protection in that and the harm that it causes of trying to get your work taken down, you're not really listened to. It's been posted without your consent, especially when it's on like bigger platforms, as well. As it's just, it's such a vast world, it's like hard to can speak to a human being in these sort of situations. And you're not really considered, you're not really seen as a worker, like this is a job for most people. And it's not really treated as such, because it's sex, basically. And so it's really, yeah, you just feel really unprotected in that in that aspect.  P35


like sometimes for the design of things I don't use them. I realised that if something's too complicated to use, my brain doesn't make the effort to use it and I just forget about it. So yeah, I think these two or three things will be like the most important for me. C9

==> notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% 
% END-TO-END ENCRYPTION %
%%%%%%%%%%%%%%%%%%%%%%%%%
% Skepticism/against P: 24, 22, 50, 40, 43, 14, 6, 23, 37

% There was a mixture of skepticism and misconception around E2EE such that large tech companies would be able to sell the data or use it for marketing purposes (P22, P14), that it could be coerced by the police (P50), belief that it didn't work or a lack of trust in teh protection  (P23, P43, P6)

% Or that even with E2EE, it doesn't prevent a receipient from saving an image P40.

% % [E2EE] Doesn't matter to me cause fb eventually sells data (P22, Pos. 392-396)

% % end to end I don't it’s useful at all
% % I don't think*	 (P24, Pos. 227-228)

% % WhatsApp supposedly also has end to end encryption. But I feel like, if someone wants the data, they will get their hands on it anyway. And if that someone is the police, for instance, they will just force companies to give that to them. No matter how well encrypted it is, so it doesn't really give me a good sense of safety or security to use end to end encryption. (P50, Pos. 274)

% % I just feel the... like WhatsApp, for example says that it has end to end encryption, but I still don't feel like WhatsApp isn't necessarily safe app. So that's why I don't really think about it.
% %  (P23, Pos. 276)

% % That's fine but you can... you can save an image and you can screenshot so. (P40, Pos. 248)
%  I do not trust it. Because the if the police needs information, they will get it. They will actually get it and if that's legal for them to do, they will. And there have been breaches, I mean, in such chats. And also, that doesn't work. The end to end encryption doesn't work when you are in a group chat. From what I heard, I'm using Telegram and it says that it's not it's working only when you're talking one with another person. (P37)


% Yes, I do. I hear it. But obviously, you still, you have to be sceptical about it. Because still, you know, it's not... They say they are end to end encrypted. And at the same time, you hear that it's like, Oh, this is still not safe. It's not completely safe, and blah, blah, blah. (P43, Pos. 312)

%  % it’s some kind of additional security but I don’t really trust WhatsApp about it. All the data is used for marketing and advertising purposes so I feel like the app for sharing intimate images shouldn’t use our data for any targeting purposes (P14, Pos. 90)

% % I'm not sure I trust it anymore. Like WhatsApp seems pretty undermined now. Originally, like that was a strength of that which should bear in mind. I guess for Instagram and such I have no idea what if they even promise you end to end encryption . P6

% Use P: 42, 38 (email and text), 8, 13, 48, 29, 39, 47, 26, 2, 51, 10, 17, 15
% Useful: 18, 12, 31, 34

% % I think it is, definitely. 
% % It probably addresses my own actual concern, which is exposure, not by an individual, but by a platform or like an infrastructure itself. So yeah, I definitely think it's useful. Yeah. (P47, Pos. 236)

% % I mean, in general, like everything that is like communication, I think it's important. Yeah. It's yeah. (P39, Pos. 262)

%  % Protection from the government and partial from police.  (P38)

% they use end to end encryption, which gives me more trust. (P13, Pos. 181)

% The only thing would be to use end to end encryption, and like to... Yeah, I can secure the communication, I can secure the storage where the photo is in, but I don't think I can prevent anyone from actually getting pictures out of themselves if they want to. (P26, Pos. 216)
%  % If I sent intimate pictures, 
%  There are basically two possible attackers. Like either the person I'm sending this to or someone from the outside trying to break into systems and stealing data. Since I want the recipient of the message to see the picture and therefore be able to leak them anyways, it's just not an attack I care about. So I leave the security there. I mostly care about somoeone from the outside able to steal pictures. And as I said, for me that scenario, like the risk that this... of this actually happening is acceptable, but in general Yeah, I would just like to see if I was... this simple security feature present on telegram. Not only for intimate pictures, but any sensitive data, which is basically all the private conversations that are happening on the platform. 

% I like to... it has to be sort of end to end encrypted, as far as I know. And it has to not be publicly accessible. And I have to... I have to be confident, well reasonably confident, that the images I send aren't being stored on some remote server that I don't know about.  (P2, Pos. 52)

% then you mentioned encryption. So to you, why would you say encryption is important? P 46:57 
% As far as I understand encryption is that it transfers, let's say, data between you and another part in a way that the data is not understandable or readable to the connecting part, let's say like...
% , understand that a certain website or certain platform or certain app is not encrypted, I would definitely be avoiding it. (P51)
 
% Because nobody knows a where from the picture who is behind the picture? You know? (P36)

% , it certainly makes me happy to know, I'm comfortable to know that it's end to end encrypted. You know, I live in the UK, which is not as monstrously evil as it might, it could be. But it still has a government that wants to access your details.
% And if there's anything I don't want, it's the government knowing details of my personal life and seeing my tits. So yeah, for sure. Yeah, like end to end encryption gets a big thumbs up from me (P10, Pos. 351)

% WhatsApp just for convenience. Sometimes, you know, you move the conversation from Grindr to WhatsApp, and then they just send them there. So that's kind of what... I understand whatsapp is now encrypted end to end anyway, which seemed quite secure to me (P17, Pos. 29)

% Yeah, I mean, for privacy, and I think because it's the most standard thing for texting, kind of taking, taking it for granted I think now, it will be suspicious if one app didn't have it. P15

%  Ambivalent
%  Sure. But as I told you, this could be important if I'm a person that someone thinks that I should be hacked, so for... I mean, for people that are common people, I would say that it's not such important end to end encryption. (P21, Pos. 248)


%  Don't care
%  Well, in my case, I don't really care. I feel like end to end encryption, like, I guess it's for more, let's say, sensitive stuff. No, maybe. Maybe you you're into like direct role play. And you wouldn't like that kind of stuff to be shared. But I don't think I really care about that when sharing like, loaded images of myself. P3

%  I don't care about the platform reading the message. P4


%  all of the Messages app that I have used have end to end encryption, I guess, but I'm not sure. I know that WhatsApp has it because when you you have the option to activate end to end encryption. This feature is thing that I assume that an app has. Yeah.
% I  33:34  
% So when you decided to use whatsapp telegram signal, they do all have end to end encryption, did you select them Because... partially because they had end to end encryption. Did that factor into your decision making? Or is it just that they happen to have end to end encryption? 
% P  34:01  
% I choose them because of other factors instead of the end of end encryption. (P19, Pos. 280-284)

%%%%%%%%%%%%%%%%
% WATERMARKING %
%%%%%%%%%%%%%%%%
% Use P: 5, 17, 27, 31. 33, 34, 35, 37, 40, 48, 50, 52, 53 (13)

% Watermarking, which is used to apply a visible (or invisible) signature to content, was mainly used by the sex workers we spoke to. Overall 13 participants used it and primarily noted that it helps with claiming ownership over content and deters others from stealing and re-selling content:
% \begin{quote}
%     % "If your content's watermarked, then other platforms won't allow it to be uploaded. And I think that's the thing we have this conversation with these collect collectives of sex workers where they just like watermark your images, watermark your images, because it provides a lot of protection. And like,
%     "If you brand yourself in a specific way, it highlights the fact that this is a service, and you have control over this service. And then other platforms where if it does get leaked, or if boundaries are crossed these platforms won't accept it, if it's been watermarked as something else, because they then know that it's not." (P35)
%     % , unless you don't have proof that this has come from that person that's been watermarked, then it won't be posted. So that's kind of reassuring, but again, can still there's still ways around that if people really want to ruin your life. Sorry, I'm being really dramatic. (P35, Pos. 237)
% \end{quote}
% Another group of people regularly using watermarks were participants who used specific gay dating apps where the platform automatically adds a watermark to uploaded images. P5, explained, 




% % I used a personalised watermark for... or a personalised icon for letting know that that's me, that's my production. But I didn't use it too much because I think I'm a pretty easy to recognise person so if someone sees my content anywhere it will be clear that it's my content artistically and visually and everything. And I don't have... the thing is that i'm not so afraid of intimity (privacy) being... I'm pretty open about myself my status, my whoreness, everything so I don't have problems with that. And it's something that I'm mentalized (aware) that can happen. P42
%  I think Grindr does that interestingly, already, I think with the images you share, I believe there's a Grindr mark in the in the corner like that.  (P17, Pos. 213)

% Nowadays I  just watermark all my content, and it's so that you can claim ownership and even when you report it and when you report on social platforms. Like you have proof of ownership. Yeah. (P53, Pos. 200)


% To make it a bit more difficult for people that collect these photos and resell them or use them in other websites just make it a bit more difficult. (P37, Pos. 169)

% I mean, I guess it sort of deters people from pretending to be the person on the photo or sort of spreading your photo as theirs, but it doesn't necessarily stop the spread. So I, yeah, I guess it's useful, but not 100\%. This app that I mentioned, Hornet, for example, has that? Yeah. When you sort of want to look at someone's picture, full screen. Everyone has this, I guess, six, seven digit user name. And it always displays the username, however, you can still it's sort of on the on the left side of the screen. So if you zoom enough, you still sort of evade the watermark, but yeah, (P5, Pos. 467)


% So like, recently, a little bit more, I've put like, texts in the images themselves. So like, when I edit them, I'll put like, a little sentence in the image not to like hide anything or to, I don't know, watermark anything, but just to sort of be like if someone would receive that they would know who it had originally been sent to. And like that it was meant for only them and so obviously, they can then see that that person has crossed a boundary. So I hope that sort of deters people from sending them on. (P31, Pos. 157)
% it shows that it's yours. And like in that way, it can become a bit of an advertisement or something. But in personal life, I think also the way I do it, it just like I think it is my way of trying to implement sort of the like, putting the accountability on the person who is sharing it instead of me. Like who's non consensually sharing it instead of me sending it so like by including their name in the image, you sort of implicate them into it more. (P31)

% Unsure/concerns: 
% And I don't know, like, part of me wants to say like to have stuff watermarked. But I also know that the process of having content taken down off the internet can also put you in more danger. So there's people, they... you have to like, let's say, nonconsensual porn of you has been uploaded, you have to sometimes provide like a photo ID and like proof that it's you. And that way it ends up identifying you and potentially putting you at even more risk because you're trying to have this thing taken down. So I think it would be really important for companies to really think about how they are going to deal with people's requests to have material taken down and what they can do to protect people. And yeah, it would be nice to have things watermarked, but that could also be used against people like, oh, it's the same girl in all these photos, collect them and put them in a folder together. (P18, Pos. 284)



% Used to use: 
% Yeah, I used to, well, it's not really something that prevents it from being shared without my permission, but at least it shows where the content is from. And for, like, some of my images, I would use my, like, social media handle or my, like, onlyfans handle to... as a watermark, but yeah, I mean, that doesn't really prevent them from being shared. (P46, Pos. 114)

%%%%%%%%%%%%%%%%%%%%
% METADATA REMOVAL %
%%%%%%%%%%%%%%%%%%%%
% Use P: C37, R26, C33, C46, R23, R10, R12
% Metadata removal is used to eliminate extra information that is added when an image is created, such as the location, date/time of creation, and/or the type of device used. Though only 6 participants used it, they generally expressed that they would prefer for it to be automatically done by a platform when an image is sent. For example, R2 expressed that, "For any intimate photo sharing app, I would hope that that would be in there by default, and it wouldn't be able to be turned off." Of the safety strategies they used, a few participants admitted that they were less strict about using it and that it is, "something that I often forget and not only forget, and sometimes not bothered to do" (C37).


% always a big fan of metadata removal. I'm just a big fan of metadata removal in general. I'm just like, don't like the idea that someone can work out where I took a picture. And because I took a picture and then like that happening. I would rather have that wiped. (P10, Pos. 439)

% Something that I often forget and not only forget, and sometimes not bothered to do is to remove the metadata from my, for my photos and videos, that's something I often forget to do. (P37, Pos. 89)
% I right click the files in my file explorer, and I think somewhere in the Properties has the option to remove the meta the meta data and some other times, um, I'm thinking that when I send a photo through a social media like Messenger, these meta data are removed any any ways before they reach the recipient. (P37, Pos. 97)

% wants in-app (46)

% Yes, I think yeah, I would say that I'd be a big plus as well. And actually, now you mentioned it, I think it would be a big negative if that turned out to not be done automatically. I think... I don't think many apps do this at all. But I would think for any intimate photo sharing app, I would hope that that would be in there by default, and it wouldn't be able to be turned off. (P2, Pos. 312)

% I think it's absolutely necessary if I post publicly. P26
% I know that the app does it. So I don't go for any... most apps. (P26, Pos. 388)

%  I was less strict about my metadata scrubbing policy (P33, Pos. 245)

%  always a big fan of metadata removal. I'm just a big fan of metadata removal in general. I'm just like, don't like the idea that someone can work out where I took a picture. And because I took a picture and then like that happening. I would rather have that wiped. (P10, Pos. 439)

% I think metadata, data wiping as well just be able to blank that aspect is pretty. I mean, 
% it pretty almost feels like that should be the default when you share any image anyway, but there's context. Again, like I wouldn't think about, like, because I don't think you don't really think about that kind of thing until you like, there's very specific situations where you start thinking about, 'Oh, well, is the image taken.' And when it's not like how we conceptualise images, we still conceptualise them as like, a photo versus rather than digital objects. (P6, Pos. 313)

% WANT MAYBE? 
% So you mentioned when you click on the photo, that you can see the information about it. This is called metadata. And some people prefer the information is there, and some people would prefer it was automatically removed. Do you have any feelings about that? Do you just leave the information there? Do you remove it, would you prefer the metadata was removed?
% P  37:51  
% I don't know how to remove it to be honest, I don't know how to remove it if I take an image. But like I said, it's been a really long while. But I... so if someone has a photo of me, it's the only way that they got it is either when I sent it to them, which probably not a really revealing photo, the second is the one time view, so they probably took a screenshot so it wouldn't really matter what kind of metadata there was. (P43, Pos. 346-348)



%  assume you'd have to be quite technologically adept to kind of use this kind of thing. If you are that kind of technology adept to use that kind of metadata, there's going to be easier ways I imagine to get your privacy data out there, essentially. So I'm in favour of having it blocked, I think for sending an image you should be sending the image, or at least it should be asked, 'Do you want to send them the meta data metadata along with this photograph?' And so if it was able to be blocked and taken off the photograph, I'd be in favour of it, I think that'd be good. Again, I think thinking about it if the person is so digitally adept to be abused that that they're going to find some way to get your nudes anyway. So it's a bit of a moot point, so wouldn't be a major priority for me. (P17, Pos. 225)

%  Also something I think about very often, but never actually do. But I know I probably should. But yeah, I think, especially with, like, risks of, you know, especially when it comes more to things like sex work, risks of doxxing and those kinds of things. It's just really helpful to have that removed. And I don't think we're all thinking about it all the time. And you kind of forget it, because it's not, it's not right there on the image, you don't see it directly, you need to like go out of your way to find it. So yeah, definitely big supporter of that. And also think I should be using it more. (P31, Pos. 261)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SCREENSHOT NOTIFICATIONS %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Use: R2, R4, R6, C9, R11, R14, R17, R18, R22, R28, R29, R30, R31, C35, C42, R43, C54, C56 (18)
Among recreational sexters, they mainly associated the feature with Snapchat and many wished to see it be more heavily integrated onto other platforms. 

"transparency"

% eople would screenshot things maybe, but you kind of know like that. There's like that violation and that happening, which is like an interesting aspect of that developing. R6

. And I think if you know that someone is notify when you are screenshot, you don't do it. Even if you want to do it, you don't do it. C9

% It definitely. Not only in talking about nudes, but it definitely did cause some fights, I think, not only with me, and you know, the people that I was interacting with, but actually the sort of the story that I mentioned about me asking a friend to delete sort of an intimate picture was also like that, because I knew that they had screenshotted it and I was like, Can you please delete your screenshot? So I guess it's it's yeah, it's the fact of and it's useful. (R5, Pos. 443)

you can still record your screen and the other person won't know it (R4)

Oh, yes. Yeah, I mean, I think those are in general, better than not having them. Because then, you know, if someone who's not super tech savvy, or like, hasn't really thought about that, screenshots, at least, you know, and you can, like, try and deal with that in a way so then that's better than not having it. But I don't think it's like, a thing that fixes everything, because there's always people who can figure out ways around it, or like, even, like, it sounds kind of stupid, but even like taking a picture of another screen with another phone, or like with another device, you won't get a notification from that ever. So like, people can still take pictures of things. (R31, Pos. 249)

 you can start to ask questions. (R28, Pos. 193)

There's also ways around that though. I remember friends saying that you could screen record without Snapchat send you a notification. R11




%%%%%%%%%%%%%%%%%%%%%%%%%
% DISAPPEARING MESSAGES %
%%%%%%%%%%%%%%%%%%%%%%%%%
% Use: R2, R4, R5, R6, R10, R11, R12,R13, R14, R15,r16, R17, R18, R21, R22, R23, C24, R26, C27, R28, R29, R30, C33, C35, C36, C39, R43, R47, R51, C54, C55, C56


% that data exists on my phone and then is sent through servers, so exists on the servers, which will keep a record just because servers can't decide not to, like even if they disappear, they don't necessarily disappear entirely. And you know, there's always a worry for me of like, well, someone could dig it out. If they were determined enough to. P10


% Use w/ stranger: R11, R12, R14
% , because I knew the person less at first or I was, you know, just starting to message them. It it did it.  R11

% Sometimes yes, if I don’t really trust the person I choose the option in which you can display the photo just for once (R14)


% Like I do like the disappearing photo feature on WhatsApp, then I feel more comfortable sending images that I might not have been comfortable sending before. R18

% think it gives you more control of what you were sharing.  C39



%%%%%%%%%%%
% VETTING %
%%%%%%%%%%%
% Use: R3, R4, 9, R12, 18, 24, 26, 33, 34, 35, 36, 39, C44, R47, C48, C49, C50, R51, C54, 

%%%%%%%%%%%%%%%%%%
% IMPLICIT TRUST %
%%%%%%%%%%%%%%%%%%
P: R2, R5,R6, R7, C9, R10, R14, R15, R16, R17, R18,R19,R21,R22,R26, R28,R29, R31, C33, C37, C40, C41, R43, C44, 
And I've never had sort of discussions of boundaries or anything beforehand. It's always been sort of a gradual feeling out of things, and never an explicit discussion. R2

so in groups, it was always groups of friends. And I feel like the trust was so established, though, I don't know if that was always correct. But like, the feeling of trust was so established that it didn't feel like you needed to say that. R31

I feel like it is implicitly implied, but I've never said to do that, never said make sure you keep our things private. C40

I just believe that this is sort of the underlying assumption or the agreements R5 

%%%%%%%%%%
% BACKUP %
%%%%%%%%%%
Cloud backups
% P: R2, R6, R13, R14, R16, R17,  C24, R26, C27, R28, R29, C35, C42, C46, C49, C53, 
% Mostly automatic!! 
% Count; 16

R17: deletes from cloud
R14: pefers not to

Ideally, it'd be great if you could kind of stop auto backup for kind of pictures when they were kind of sent, because then essentially could just save me the hassle of going in and deleting them, essentially.  (R17, Pos. 189)



I tend to... I mean, I try to generally avoid the big, like, the big corporate cloud storages, even though it's a bit impossible these days. For example, my photos, my videos in general, I don't back them up on my Google Cloud or whatever. However, I do sometimes back them up on my computer, but that's a bit... It's not very systematic.
 (R47, Pos. 12)


%%%%%%%%%%%%%%%%%%%%
% SECURITY FATIGUE %
%%%%%%%%%%%%%%%%%%%%
I  15:45  
And are there any strategies that you use to try and avoid risks of storing? Or you feel... you know, you do what you can?
P  15:57  
I do what I can. And besides that, I just think... I just sometimes think it's pointless, because all of my pictures and all of my info is like, already there. So I don't know why I would bother any further.
 (R23, Pos. 193-196)

% \lucy{quote already mentioned}

"Mainly because I find tech stuff pretty, like overwhelming. I mean, I'm tech savvy, but like, just the sheer amount of content that you need to produce. Like, kind of stresses me the fuck out. So I was just kind of using the easiest. [...] I have not been very cautious about the way I store my images." (C46)


"I'm pretty bad at keeping my security. I have everything stored everywhere, I have it in my phone, I have it in my harddrive. I have some parts on the cloud in some places, and in others, and sometimes I forgot where were the things so I'm pretty bad at giving security and accounts of where all my work is and how its secured." (C42)

I kind of not give the right importance of security anymore. It's like I gave up my security of the... like how I could prevent something to happen. I also realised that I don't have the knowledge, everything I have read, it seems too complicated.  (C9, Pos. 124)



I sometimes feel I spend more time scrubbing personal info off my pictures, putting them in private folders, etc. than actually taking said pictures
the learning curve is steep when you want to do things well.
(C33, Pos. 122-123)

% ADDITIONAL
I'm pretty bad at keeping my security. I have everything stored everywhere, I have it in my phone, I have it in my harddrive. I have some parts on the cloud in some places, and in others, and sometimes I forgot where were the things so I'm pretty bad at giving security and accounts of where all my work is and how its secured. (P42, Pos. 20)


Mainly because I find tech stuff pretty, like overwhelming. I mean, I'm tech savvy, but like, just the sheer amount of content that you need to produce. Like, kind of stresses me the fuck out. So I was just kind of using the easiest. I hate like, I haven't produced videos in the last like, six months maybe. But yeah, I have not been very cautious about the way I store my images. (P46, Pos. 32)

 And I'm a bit too... I'm quite laissez faire with it. I'm just hoping I will... this will not target me, but maybe that's wishful thinking.  (P50, Pos. 112)


% HAPHAZARD SECURITY:
Yeah, putting these images in certain hidden folders on my phone, for example, and also just sort of deleting ones where they are... deleting ones where they appear and sort of... I guess, it's kind of random actually. It's not very systematic, but I guess sometimes I will think, oh, there's sort of a patch of nudes in the gallery around through this day last week, which I've likely to scroll past it'll be obvious what they are.  (P2, Pos. 188)

I think about it sometimes, like what would happen if my colleagues at the University were sent a bunch of naked photos of me? And like, how would they react? And I would like to think that it would be a non issue, and instead, the focus will be on the person who was non consensually sharing images of me. But unfortunately, there is a lot of victim blaming around this. Like, why did you share these photos if you didn't want other people to see them? So sometimes, I do feel like maybe I shouldn't be doing this. But then the other part of me is like, fuck the rest of the world. I'm having fun. I'm an adult. I want to have these kinds of conversations with people and I don't want to allow shame or stigma to prevent me from living my life and exploring my sexuality as much as I want. [P18]

No, and I'm a bit... I'm not, technology doesn't interest me that much. For me to do a deep dive in a good application seems a bit like a stretch, I want to have sort of take the easiest route to... (P50, Pos. 104)


Watermarks. I'm also not... I'm just, I'm too lazy to bother lots of the time. And I like onlyfans, because it puts watermarks there automatically. And I don't have to bother with my editing software. (P50)

Something that I often forget and not only forget, and sometimes not bothered to do is to remove the metadata from my, for my photos and videos, that's something I often forget to do. P37

% Ppl who don't like any apps:
Not really, I don't like them really much so it's complicated for me to...  (P27, Pos. 195-196)


Watermarks. I'm also not... I'm just, I'm too lazy to bother lots of the time. And I like onlyfans, because it puts watermarks there automatically. And I don't have to bother with my editing software. (P50)


And I think probably not, because, you know, it's not something that I do. It's something that I kind of only do on the spur of the moment, I don't plan to do it. So there is no reason why I would need a specific platform for it. And also, it's not something I do with people that I don't already know quite well and trust a lot.  (P29, Pos. 56) 


the learning curve is steep when you want to do things well. I feel being tech savvy helped also (P33, Pos. 123)

to be aware of new kind of advice that's coming out, because technology changes so fast. I can't keep up. P29

Something that I often forget and not only forget, and sometimes not bothered to do is to remove the metadata from my, for my photos and videos, that's something I often forget to do. P37

I think I'm not as diligent with the intimate content as I am with other types of content. So.
I  17:41  
Okay, yeah. Would you mind speaking more about like, what other types of content you feel that you are, I guess, a bit more diligent with?
P  17:50  
So definitely things like, yeah, card bank details. My personal identifying details, let's say like, ID, social security numbers. Yeah, I guess, these are definitely things that I'm trying to be careful with, mine or others, because I might also sometimes handle others' details digitally. And I'm trying to be careful with that or with data that has to do with my work. Cuz sometimes I work even on my private computer on things that are related to my job. So then I will also try to be really careful with that. (P47, Pos. 104-108)





%%%%%%%%%%%%%%%%%%%%%%%%%
% UNINTENTIONAL CONTENT %
%%%%%%%%%%%%%%%%%%%%%%%%%
STORAGE-BASED:
P: R2, R3,R6, R10, 13 53, 4, 6, 8, 29, 17, 31, 48, 22

I just wouldn't like for someone to just stumble on my content on my laptop (C53)

I knew they wouldn't look for things but it made me uncomfortable knowing they could find content by accident, so extra precaution C48

 No one wants to kind of come across that for that on their friend's phone. Which is why I think this has opened up to position it in a different place. R6

 Honestly, I delete them pretty fast, just because there's always that anxiety. 'Oh, God, what if I accidentally send', I'm trying to send one image to a friend that actually sent this one I'm probably going to leave that instead. (R10, Pos. 171)

 there is always the risk that I might lose my phone or I might lend it to somebody, and they might accidentally see something. You know, if, for example, if I'm sitting next to my friend and I'm looking through my camera roll and they happen to glance over and see, like naked pictures of me, they haven't consented to see that. You know? That's the kind of... that is a situation where I feel like I would be... (29)
 
 Yes, I guess the risks of it potentially being leaked, or accessed by other people, or the risk of it, accidentally displaying on my phone in, in a dangerous context. So eg if I was trying to find a photo of like, a Wi Fi password at work, and I accidentally scrolled past some intimate images, that's probably the danger I'm most concerned with.  (R2, Pos. 184)

DEVICE SHARING:

	I have cousins, my mom, my grandma
19:47:17 P
	yeah
19:47:30 P
	they can take my phone anytime and browse gallery
19:47:37 P
	also they take photos
19:47:42 P
	and check them (R22, Pos. 290-298)

I suppose the main one is like, the accidental access by other people. So like other people who will occasionally be like using my phone or my devices for? And in order to quickly set a timer or change the song or like, there's kind of like some sorts of it's not a completely private device, the way I use it. R6
many of my friends probably would know my password and could access my phone if they wanted  R6

% SHOULDER SURFING: 2, 6, 11, 12, 16
% Just because I've heard a lot of stories from friends about, well, I've heard a lot of stories, just sort of people, friends sitting next to me, and like a horrible picture pops up on their phone out of nowhere. So I think it's just generally reactive, I think, sort of responding to tone is the kind of context that would get me to send an intimate image. (R2, Pos. 100)

% The other thing is also like in a whatsapp rule. So I was one a while ago when I think my partner shot the photo was just kind of in our reel but then it's like, because we hadn't sent more messages every time you kinda open the phone around that that would be the visible image on the screen, which is inconvenient in a more public setting. So I shouldn't be like delete that because the message was deleted to remove it from the reel before. So that's like a Yeah. Another kind of story of I suppose this chat log storage? P6

% have I been concerned that someone has accidentally seen a photo because I've sent it at the wrong time? 100\% I have believed that has happened.  P11

% , 'hey, you know, is it like, is this good time or whatever', or if I send it, I will then also sometimes, if I'm unsure, like, couldn't get like a response, then I'll like very quickly send like a bunch of texts, like text based messages below to kind of like bump it up, so that it wouldn't necessarily be the first thing that comes up on a screen when he opens something, for example P12

% That someone else beside the person I'm sending the content to might see it, whether it's in the moment if he's in good company, or later on will share it with other people. (R16, Pos. 188)

% THEFT/LOSS: 
% P: 21, 28, 30, 49, 51, 29, 16

% I'm not sure. Like, if someone would steal my phone I think it wouldn't be so safe for me. Like I forget the word. Like I would forget my phone from somewhere and someone took it, it wouldn't be safe because I don't have any passwords. I mean, I have but I don't think it's very safe password to my phone. (C49, Pos. 36)

% And there is that I get my phone stolen, which happens at some periods. And that's someone like could crack my code and take my pictures.  P30

% I have considered what would happen if my hard drive or my computer were taken. I have biometric security on that. But I just tend to be really safe with it.  P40

%%%%%%%%%%%
% HACKING % 
%%%%%%%%%%%
P: 5, 8, 9, 11, 12, 14, 16, 17, 19, 22, 23, 26, 30, 34, 35, 38, 45, 55, 56 
count: 19
Viruses, phishing

my Contact was broken into, it's not as inconvenient to me, it's dangerous to others. Because that I use, obviously, I mean, obviously second, like two factor authentication, but also Password Manager. Autogenerated, very long passwords that I change regularly, stuff like that. So this is my top security thing, is precisely because of the things in conversations that I'm worried about. P7



But I also have thought about it, like have had nightmares, but I also don't understand how hacking works. R11

COMPANIES HOLDING ONTO DATA: 

%%%%%%%%%%%%%%%%%%%%%%%%
% POSITIVE EXPERIENCES %
%%%%%%%%%%%%%%%%%%%%%%%%
 So like a rampage of trampiness. And it's been absolutely amazing. And so at this point, I'm exploring a lot more kinks and fetishes that I didn't have the opportunity to explore before because I was married, in a marriage, and then also pandemic. And so after, like seven years, I'm finally maybe even longer, I'm finally able to do whatever the fuck I want. And it's great. And I'm having a great time. But there is that concern that... it's not even the images that worry me, it's the text messages that I think would be of greater concern to me.  (R18, Pos. 232)

%%%%%%%
% IIA %
%%%%%%%
WHO:
I assume they're probably being shared. And I mean, ideally, I would prefer not. And if they are shared, hopefully, in a positive way, not like, look at this dumb bitch but look how hot this girl is. (R18, Pos. 224)
let's say, I have a boyfriend again someday. And he decides to look at my laptop or is curious about what's ever on my external hard drives, or I have a lot of physical copies of nude photos, it would be very easy to take pictures of and you know, text to people.  (R18, Pos. 268)

Yeah, I think, like now that I have almost no control over my image anymore, not only because of porn, but because also I have done activism and given interviews where (inauduble) the interviews, but they're out there on YouTube and have, like 1000 views.  (C9, Pos. 248)

I wouldn't be surprised if some picture of me was also shared. And like I said, it's... in those male context, in the context of like group chats it was definitely shared outside. And God knows where it has been but I've never been notified about it. So I've never looked at it. (R7, Pos. 240)

Um, I do have some concerns, but it's about the clients usually and the people I interact with, not actually the platforms, um, I'm sometimes worried, whether they're asking for pictures just to collect them and use them or sell them.  (C37, Pos. 217)

% Was also worried that these videos are distributed by whatsapp groups or telegram groups because I know there are groups on telegram and WhatsApp where people send porn. And then you don't have any control over it. You don't even know them. Because if you're not part of these groups, you don't know how they're there. And sometimes I have my videos also leak on Twitter. And even if I report them, I don't get them deleted. So this was also a big concern, that my videos that are intended for people that are paying, and that there is less people are being seen for free in platforms that I didn't choose. (C9, Pos. 140)
 
I imagined certainly the people I've sent them to have shown their friends, for example, or in passing around like groups kind of trading nudes, I imagine. None of which I've done but imagine does happen. So I'd be very surprised if my nudes hadn't been shared in some way, shape, or form. But nothing publishing has gotten back to me. So yeah, nothing causing me concern. (R17, Pos. 245)

Less concerned: 
Yeah. No, very rarely I have felt actual worry that they will do it willingly and consciously. (R47, Pos. 196)

Yeah, I had it in My previous relationship, and before I started this work. Now I am more... there are pictures of me online are ready. So if somebody's going to post it, I wouldn't be very happy about it, and it will be disappointing. But on the other hand, let's say I don't feel threatened by it so much as before. And I also realised how many intimate pictures and how much content, this style content, is online and in the past, I really thought if there would be a picture, like somewhere of me, everybody's gonna know. (inaudible) is gonna recognise me and now I realise it's a lot of work to even get seen and get recognised somewhere. So yeah, and now, obviously, if I send something privately, I'm just aware to who. And if I trust this person, but if it's gonna leak, yeah, I'm not that afraid anymore. (C52, Pos. 392)


 Everyone does it. Everyone does it in relationships. No one really cares for security that... I mean, there's obviously like, don't send it to everyone, obviously. But even during like the hookups and stuff, people do it. And so I guess maybe I was... I had no, I was never really too concerned because nothing bad ever really happened. So no. And obviously, we didn't talk about harassment. Obviously, neither me nor my friends ere ever harassed because of stuff like this. So no. (R7, Pos. 160)

even though these people were shitty people, they're not so shitty to fuck up my life. They're just kind of emotionally dumb. And therefore, I don't think they would do something like that. (R11, Pos. 165)

I don't even if I've stopped dating them or something like that, I don't think just because of who they are. That's that's the sort of thing that they would do. Yeah. (R12, Pos. 137)

Yeah, yeah, exactly. I would say the only risk would be like something clumsily ending up in someone else's device or, you know, I generally don't think that any of these people that I've had personal relationships with are getting up to anything nefarious with my images. (C46, Pos. 290)


I just, I have so many people's nudes, that I feel like if they tried that, it's like, what are we going to do, like quid pro quo babe? Like, it's like, you kinda post my shit unconsentually, and and what I post your shit unconsentually? Like, what? What are we doing?  

% Yeah, I talked about that. And I saw pictures that I could send to my lovers. So it would be stressful for me, but I take the risk.
%  (C49, Pos. 164)

More concerned: P21 (didn't quite understand what they were articulating)
Well, I have general concerns about all these things. I heard all kinds of stories about revenge porn and these kind of things that I'm concerned about if someone might want to have bad feelings about me after things end, and for some reason, decides to use intimate pictures of me for any reason. (R16, Pos. 196)

I am trying not to think about that kind of stuff. Because after that, I'm starting to be afraid, you know that somebody can do something like that for me. And that's why I like to really, like I'm really patient with choosing my clients. And I have to talk with them a lot to be sure that we can meet and nothing bad will happen like that, you know? (C54, Pos. 108)

I think it's really isolating when work is shared without your consent, when you send it to a client, and that's been shared onto another platform without your consent. There's no question that when it gets to that stage, there's no control over it. (C35, Pos. 185)

Yeah, I'm afraid that the content will be shared without my permission further.
 (R45, Pos. 313)

plus, I'm using a VPN everytime I log in on my platforms
because even before becoming a sWorker, I was aware of the risks of keeping sensitive content on my device + I heard many things about revenge porn, hacking devices and stuff like that
one of my priority is safety (C34, Pos. 34)

I mean, because I worry more, I don't send that like, super explicit things (C44, Pos. 380)

That is, that is totally where most of my anxiety, like again, not crazy like it, I very much try not to be too paranoid. Because I can't control other people. All I can do is control myself and what I do. (C38, Pos. 337)


Stories of life destroyed because of that. You, yeah, I think about it all the time. When I when I send them (R30, Pos. 89)

I think about it sometimes, like what would happen if my colleagues at the University were sent a bunch of naked photos of me? And like, how would they react? And I would like to think that it would be a non issue, and instead, the focus will be on the person who was non consensually sharing images of me. But unfortunately, there is a lot of victim blaming around this. (R18, Pos. 228)

Societal norms:
Yes there would be repercussions from my family because even if I live in Europe, I was born in Turkey and Turkey is a very conservative and traditional country. My parents are open minded but I don’t think they could handle this fact (R14, Pos. 59)

perhaps in the gay community, more so than the straight community um I think it's less embarrassing. You know, I'm sure I must have seen a lot of my friends nudes, for example, in through scrolling, things like that. And it's kind of funny, to be honest, you know. I imagine for other people who'd be a bit more conscious of it, and perhaps a bit more worried about that social embarassment factor it would be more of a risk. (P17)

I always feel like it's always women who have to worry about that and everything. Like men, I think for a lot of men, the question is not even even they don't even worry about it, because they don't really care if there is a dick pic in nature or anything. (R30, Pos. 253)

I think there was a lot of shame, particularly for maybe cisgender women. Like, it's like, "oh, people are gonna think I'm a slut". And I'm like, and what about it? Like, you know, like, but at the same time, those kind of consequences are much more real for cisgender women who are not sex workers, right? Versus, you know, like, I'm gay, man. Like, it's like, it's, you know, yourself, like gay male culture is sucking and fucking, like, oh, he's a slut, oh, no! That's gonna make me more popular at the bath house.  (C38, Pos. 185)

in an absolutely ideal world, this would not be a possible threat: I think it has a lot to do with patriarchy and how sex equals degradation for women (C33, Pos. 331)

the way that I conduct my relationships is non monogamous, and I have sexual partners of all genders. And it's... it would just, I know that there are differences in how people conduct their relationships in the queer community versus the majority heterosexual community. And, you know, there are different implications with sharing intimate things with heterosexual couples and with queer people. Yeah, it's just kind of sociologically interesting to me. 

there's probably a difference between women in a straight relationship sending photos than there is to gay men, where, you know, the kind of level of physical vulnerability isn't there for well, isn't always there for gay men, let's say. So I think there is probably differences between sending it and the kind of social norms of the gay society, there are nudes everywhere, I've seen as I said, many my friends naked were I imagin a lot of straight couples, for example, haven't  (R17, Pos. 177)

I tried to be mindful, but I'm not altogether that concerned because, you know, to a certain extent, it's already kind of, like, widely known that, you know, I, you know, I'm a non monogamous person that I date, really extensively, you know, even like, you know, my family members and stuff. So, if my were intimate things of mine ever to leak in a particular way, it would just be full- (R12, Pos. 85)

it was also different as I was working as a girl and was posting more vanilla content I've the feeling that there is a facility to share content made by women because it’s also a way to show that at the end men are in control (or at least they want to believe they are), I don't think it's only related to having free pictures/videos. (C41, Pos. 69) (non-binary perspective)


Yeah, yeah. And it would be like, well, what are you going to do? And they'd be like, and I wouldn't be happy about it. Like, to be clear, I would be you know, upset by that, obviously, but it wouldn't like, bring down my career, it wouldn't get my parents mad at me, you know, like maybe it would upset my Catholic aunt but you know, I don't really care. So yeah, (R12, Pos. 89)
% Ex:
% So it was a very messy breakup, and with someone else that I trusted, so there's always whilst in my head, I'm pretty sure that that that she hasn't, there's always that bit of my head that's like, well, the archive's still there of those photos.  (R10, Pos. 131)

%  I asked him to delete all my intimate images and videos, but I don’t know if he really did because we had a hard break up. My only concern was that he might share them with my family and as my family knows my body, it doesn’t really matter if the images are anonymous
%  (R14, Pos. 55-56)

Being identified:
% Yeah, for example being linked back to me or being leaked. Yes. P43

Background fear/passive P: 5, 7, 10
 we all sort of send and receive such photos. So I try not to stress out too much about it. (R5, Pos. 233)

 ike super unlikely, just someone really wanting to find it and I don't know, spying on me about my contraseñas, My passwords, you know. No, no, I mean, sometimes, as I said, in the dark hours of the night, yeah. Sometimes I feel like, oh, shit, maybe. I don't know, whatever thing that you don't expect. Maybe what if they, like, maybe one day I'm famous or something like that, you know? And then these pictures are gonna go... are gonna show you know, like. If I'm, I don't know, like, the president of the government, and you know, I mean, whatever, or something like this, something public. What if they come, but I'm kind of part of this artistic scene, that we do sexting and I don't know, I guess I will be able to manage the situation of my worst nightmare that is that, so that's, I don't know. (C44, Pos. 172)


 But yeah, sometimes I can be a bit concerned about it, like, I can have a bit of that moment before you fall asleep, really like Oh, shit, like, all of this is out there. And then you have a bit of a panic, but most of the time, I would say I feel relatively confident that like, if it does come out, I, I would like to, like, deal with it in a way that I find suitable and like not try to not have shame about it, even though people may might want to shame me for it. (R31, Pos. 153)

Resignation:
I gave up of the idea of having videos of me that I don't like on the internet or images. I just live with that. And I don't think it's easy, but I don't know, it just... like the rules of the internet are really not nice for people selling content and yeah, C9

So that's why I kind of like I try not to focus too, because it's also like, I don't want to live in paranoia. Like I really don't I don't think that's healthy for me. I don't think that's sustainable. Because people are gonna fuck up and do weird shit anyways. 

I mean, I'm... yeah, I'm always aware of the risk that contents can be copied and put up somewhere else. But yeah, more than just sort of having an awareness of that. But I (inaudible) consequences of knowing that. (C50, Pos. 230)
I think I've become easier. Like I think I was very concerned with privacy when I first started and very quickly, I had this idea of like, okay, well, now it's online anyway. So, yes, none of it really matters anymore. (C50, Pos. 258)

OTHER:
I'm worried about the mistakes I've made in the past that cannot be undone when I uploaded something in a platform that I do not trust anymore. And I feel that I can do nothing about it. That's womething that worries me a bit. (C37, Pos. 405)

You know, everything must be, you know, viewed through the lens of the hell site, we all the hell world we all live in nowadays. Every decision comes with the knowledge that it will be observed by someone.  (R10, Pos. 467)

When I store content, I think the most risky things now for me, it's if people stole me, that is not that big of a problem because as I said before, I am pretty... I'm pretty accepting that. But I think the most problem is if I had something exclusively in one website and in some moment in the near future that website close.
 (C42, Pos. 166)
 That's my thing, my most... the thing that I'm most hesitant, or that website changed something and I lost  control of my account or something like that. Something like that, like losing... because I have some content that I... for, to making space in my harddrive I only keep it on websites. (C42, Pos. 170)
 
I have some issues but they are more like in the same direction that everything is in now in the internet that it's the thing with the cookies and all of that, with everything that the system stores...And it's the same problem for for this. I don't know until what point that can interfere with maybe I don't know like, like now there's this thing of the of the bad called AIs that make art but they aren't AIs and they don't make art, but they stole visual reference from art designers. And I think that can happen to me at some point with this thing, so (C42, Pos. 206)

I suppose. Mainly, that I just don't know like the future of like... the future of things, you know. Like that's my main concern is the tech developments and like, content that I have created over the years and this becoming kind of more accessible as time goes by. Or you know, like privacy settings changing for like a site that maybe I even forgot that I uploaded my images to or Yeah, or even just like maybe like a former workplace there may be tagged in a photo or something, then using that photo in a public context, like... because that's happened to my friend before. And yeah, yeah. (C46, Pos. 174)


REDUCE STIGMA: 
Yeah. To be honest, I think it should be part of like sex and relationships education in schools that you know, people are talking about this kind of, you know, what is porn? What is nudes? You know, how these are these things are shared, I think, would be a good idea to have in schools for sure. (R8, Pos. 379)

My concerns are about the rules of society because people act like it’s the end of the world when the intimate images of someone is leaked, I feel like the world needs to evolve 


I really hope that culture starts to change and I think that enough people are sending sexually explicit messages that like, you know, our next generation of politicians will all have nudes in the world. So hopefully it won't be a scandal. People will just be like, hey, nice tits, great. Like, great cum shot well done, and then get on with their lives and have it not be this kind of destructive force. (R18, Pos. 248)

part of me is like, this shouldn't be a problem. Like it shouldn't be a problem that those images exist. So then sort of from a slightly like, political motivation or something, I'm like, well, it's fine. Like, why why should this be an issue? (R31, Pos. 121)

I think that people in general being really taken advantage of by tech companies. [...] Like, I think that people deserve to be protected and to be able to speak freely with people in an intimate and safe way. (R18, Pos. 288)

I don't think there is a 100\% feasible way to prevent people from storing your content even if you do not give any permission to it; I think what should really be improved is workers rights and the legislation in general (C24, Pos. 211)

I would like to change society, not a platform.  (C49, Pos. 224)
When you... maybe one thing. I mean, I feel so much safer about my nudes when I think about how many people send nudes. And I think I'm, I became more confident about that. When I became a feminist, I guess, I'm gonna say, because now I don't feel that I have to be ashamed of pictures. But I would be probably ashamed when it would be stolen. But from logical thinking, I don't think I should be. (C49, Pos. 354)

I very much don't, you know, I believe in prison abolition and police abolition. So it's kind of like, I don't want to add more of the criminal system. There has to be I feel like, for me, the idea of like, people not stealing content and not sharing without consent, I feel like it's more of an ideological thing. And I feel like that's like, it's more important to talk about these things, rather than like rather than make it punitive, rather than make that it's like, like, you shouldn't do this, because you're going to get, you're gonna go to jail. I think it should be like, You shouldn't do this, because it's shitty, this is a really fucked up thing to do. You know, I feel like we should get into a place of cultural where like, if I send you a picture of my dick, and you show it to someone else, they're like, did they fucking consent to that, but they say it was okay for you to show to other people? Because I'm an exhibitionist. Right? And so it's like, if I have a lover, and the two of us are very slutty, I don't care if he shows my parts, but it's like, you know what I mean, so it has to be ideological. And rather than punitive, but it's but I understand that at the current in the current moment, that it's kind of like what we have and what people rely on. So yeah, I mean, like, having a copyright would be good. So at least like, you know, if you're really harmed by somebody, and it's to, you know, get your money, right, absolutely. Like Mia Khalifa, like poor thing. Like she got like, shit. (C38, Pos. 225)



%%%%%%%%%%%%%%%%
% Advice Given %
%%%%%%%%%%%%%%%%
Police P: 2, 8, 13, 15, 16, 19, 23, 24, 30

Cybercrime prevention unit: 22,
It's really difficult one, I know that there is a branch of the police that is there for cybercrime. But I also know that the police are not a good resource for many people for many reasons (R29, Pos. 220)


Ignore P: 2

Legal P: 2, 10, 11, 14, 22, 26, 34

Org: 14, 

StopNCII:  I don't exactly know if Facebook still has the service where you can upload a picture and ask them to remove that. (R26, Pos. 428)

"Own them publicly" P: 2, 7, 12
my general advice would be to embrace it and move on. Because there's nothing really you can do. (R7, Pos. 232)

So I guess that a lot of my advice would be about getting out in front of it and kind of trying to kind of stymie whether or not it can be used in a harmful way. And I think that, you know, that advice there would also be because I think a lot of what I tried to do when I hear about these things happen is try to turn it into a thing where, you know, underline the fact that the other person is doing something wrong. You haven't done anything wrong, they're doing something wrong. It's always better, I think, to just kind of like reiterate that. Yeah.
 % (R12, Pos. 277)

Online groups P: 10, 
% And also there are online groups who can support you in this. (R10, Pos. 443)
Screenshot proof of nonconsensual sharing: 23, 

Unsure: 6, 17

Talk to friends/family: 30

Look for advice online: 17

Confront sender: 13, 14, 16, 30, 

Report/remove from internet: 3, 13, 16, 17, 22. 24, 26, 34,
there's some pages, like in Twitter, you should be able to report the image, like there are some pages that allows you to report the images. The problem is, it's not 100\% sure that it will just solve the problem. There's my aggregator pages that just get images from this page or this page, and another page and just post them again. So it's a really bad problem. I'm not really sure what my advice would be in that type of situation.  

Abstinence: 17

Delete any content recipient can still access: 19

Other: 
I honestly cannot imagine you're going to the police with this stuff in Russia. I think they would just laugh at you.   P7

But I don't think I'd go to the police as such, though I'm not really sure where else you kind of go  P17

%%%%%%%%
% NEWS %
%%%%%%%%
% I mean, I don't remember the exact reason why. I just remember that, it could be multiple reasons over time, you know, you hear stuff, you read some news, you see things, or... It was not really one, like, reason that jumped on my face, like, Oh, now we have to delete them all from the cloud. No, I just over the years, I felt more safe. Like, okay, it felt safer that I should not keep my stuff on the cloud. (R43, Pos. 256)

%%%%%%%%%%%%%%%%%%%%%
% PERSONAL DELETION %
%%%%%%%%%%%%%%%%%%%%%
P: 2, 5, 13, 14, 16, 21, 23, 29, 30, 37, 40, 43, 49, 50, 53, 55
% Oh, hey, you better delete that stuff if you're sending your phone in to get repaired. But it wasn't sort of like a serious like, hey, please make sure you do this. R2


Yes, I did. When a partner changed his phone then I asked him to delete everything, and make sure it doesn't roll on to someone random. (16)

After breakup (14, 18, 23, 26, 30, 43, 49, 50)

Mainly in personal life for SW

Client (40, 53)

Yes, I have. Maybe when I sent them something that I later reconsidered. And I wasn't okay with sharing it. So I have a few times. And it's usually when someone requests you to send them something on their DMS, some things that I'm not comfortable with sharing. So yes, I have asked like a client about it. And he was okay with deleting it. And he promised me that he would. (C56, Pos. 261)

there was one partner who had a lot of my erotic content stored on his  computer and I, after we broke up, I asked him to delete all of it. And he said that he did. And I trust that indeed, he did. So there was some that felt like emotionally charged for a period that I wasn't sure. But by now, I really trust that he did. And there was another instance with more casual partners where I asked this because they took photos of me and then I think the day after, I didn't feel very comfortable with that anymore. And I asked them to delete it and they said they did and then later on, like months later, one of them very threateningly send me a photo. (C50, Pos. 182)

No. He was like, I've already sent you the money. And yeah, it was like, this transaction has already been completed. And yeah, I even offered to like refund but no, he didn't. (C53, Pos. 248)

one man showed me pictures of his ex girlfriend, her nude pictures. And after that I didn't feel safe. Yeah. So I asked him to delete my pictures C49

% because of the nature of my relationships being quite, you know, specifically sexually oriented and a lot of the times like, transitory in nature, like, it doesn't necessarily bother me, that like someone that I had sex with has like a picture of my boobs or something. I'm just like, 'good, like good luck to you'. If it really means that much to you, go ahead and keep it, you know, yeah. (R12, Pos. 153)




%%%%%%%%%%%%%%%%%%%%%%%
% STORAGE PREFERENCES %
%%%%%%%%%%%%%%%%%%%%%%%
Don't care: R3

Agreement with client: C55 (only those who pay for exclusive photos C53)

Once it's been sold I considered it belonged to them for personal use (C48, Pos. 151)

that was part of service. So yeah, it's something that I just accept. (C39, Pos. 162)

More clarifications around storage and deletion.

my partner does. And I think that's fine for as long as we're in a relationship of again, the expectation that on that ending, they would delete them. (R6, Pos. 161)

%%%%%%%%%%%
% GALLERY %
%%%%%%%%%%%
I guess... I mean, thinking purely in terms of what I get out of it, and what other people might get out of it differently, I think one that would have sort of different modes of... I guess, one that was less sort of, I'm sending you a picture right now and more sort of, here's a gallery you can browse, if that makes sense. So, here's my here's my intimate photo gallery with with fun annotations. Here, go in and give me your feedback. I don't know, something that made it more I guess, more playful and less sort of... Less sort of high pressure and directed like, hey, here is one image I want you to look at right now. Something that gave a bit more agency to the other person because I think there's an element of sort of exhibition to it and I think that can be more of a passive thing.
 (R2, Pos. 256)

 I'd love to have a second album on Grindr, one album for my face and my body, one album for my nudes. P3

 I have never seen any app, or I mean, or any social network that would allow you to like, you know, sort of create a photo album inside of your conversation. And that would be a killer feature. But I never saw it. R7


 There is a feature that is already being used that I think helps a bit. Some platforms have albums of photos that are not public. So when you decide to share some photos, you share that album with them that's already uploaded to the platform. I think that actually works as a safety measure because when you're talking with a client, you sometimes get carried away or you get manipulated or you are in a hurry. So having already selected part of your pictures already uploaded at a time where you are not stressed, will keep you from choosing a photo where maybe some of your personal life story, parts of your house or something That might help.  (C37, Pos. 285)

R4 wants wider adoption of album.

 organising the material sort of like a portfolio like (C39, Pos. 246)

==> storing.tex <==

\section{Storing: Technologies, Threats, \& Defenses}
\label{sec:storing}
While our focus is on the sharing of intimate images, we first asked about participants' behaviors around storing their own intimate content as it was often a first step prior to sharing. 
% We describe the technologies our participants used for storage, the threats they conceptualized, and their strategies for mitigating those threats.
%\lucy{@Elissa, this section is a bit of a mess, i'm not sure if this is the best way to organize or what should go in 5.1}

%Although the bulk of interviews were centered around participants' behaviors surrounding how they shared intimate content, we also asked questions about how they store intimate content, which we detail in this section. 
%%%%%%%%%%%%%%%%
% TECHNOLOGIES %
%%%%%%%%%%%%%%%%
\subsection{Technologies}
%\elissa{I don't mention in app storage yet b/c i think it wasn't mentioned in the original -- add something somewhere to explain, probably in the first paragraph on convenience}
% Ppl who don't use local storage: 4, 13, 15 (doesn't store), 19, 28, 
With the exception of 5 participants, nearly all stored intimate content locally within the photo gallery of their mobile device
% (38), 
or on a laptop or desktop computer. 
% (18), 
Less commonly, they used
% including in one case 
a family member's PC (R22), a external hard-drive (R15), a flash-drive (C56) or an SD card (R43). More than half of participants
% (31) 
explicitly and intentionally stored their content in a cloud/file share platform, either as a backup or primary storage mechanism. Finally, a few participants mentioned storing their images in an app (typically one they used for sharing them)
% (5) 
or in one case a photo vault app (C43). The vast majority of participants used multiple forms of storage such as C42, ``I have everything stored everywhere, I have it in my phone, I have it in my hard-drive. I have some parts on the cloud." Although, some chose only one method due to the constraints detailed below and one participant chose not to store any intimate content.
% Alternative quote:
% It's all on my phone, my laptop, hard drive, everywhere. (P35, Pos. 21)
%\elissa{note to me, come back and move this to strategies} an encrypted folder on a laptop (R8)
%Sex worker participants in particular, tended to share larger files so they more often used hard-drives, laptop/computers, and cloud platforms.
%\lucy{@Elissa, we didn't explicitly ask about in-app storage so the number is probably higher than reported. for cloud storage, did not include ppl who say they check cloud to delete images that get automatically uploaded. in section below, didn't add a count for \# of people who create on phones bc we only asked SW participants this question}

\subsection{Technology Selection: Heuristics}
Participants chose their storage methods based on convenience, technical constraints (e.g., file size), and security/privacy concerns. 
%
%\lucy{Will we need to go back and do counts for these?} \elissa{eh no i think it's not core content}
%
%\smallskip
%\noindent\textbf{Convenience.} %Storing photos in a mobile device photo gallery offers convenience for storage and sharing. 
A majority of participants used their mobile devices to capture images, which were automatically stored, 
% by the device in the photo gallery, 
enabling convenient and easy sharing.
% , which participants did primarily via their mobile devices. 
Participants also used cloud storage for convenience since %Commonly cloud storage (16) was used as a backup storage method. 
% they use ``[\textit{cloud storage,}] 
``it's automatic. I don't have to do anything" (R16). 
% Super nice...So that's mainly why I use it...convenience.'' 
%
%\smallskip
% P: 13
%\noindent\textbf{Technical Constraints.} 
Especially for sex working participants who tended to store more and larger files, cloud and file share platforms, for some, were a primary storage location and sharing mechanism due to technical constraints on the storage and speed of sharing large files through other mechanisms. 

%:
\begin{comment}\begin{quote} ``If somebody would like to buy a video, but they don't want to go to [\textit{an adult content platform}]. Then I upload it on [\textit{a file share platform}], and I share the link with them after the payment.'' (C52)
\end{quote}
\end{comment}
%
%\smallskip
%\noindent\textbf{Security and Privacy.}
% \elissa{something like: some people chose local only b/c blah; some people turn off cloud backup or explictly don't to cloud; but then there's this tension.}
% \elissa{as I indicate below, move the stuff you have under local storage in threats up here}
Finally, due to the threats highlighted in Section \ref{subsect:storage-threats} and general security/privacy concerns, several participants chose to use local data storage solutions or disabled automatic backups. C6 explains: 
\begin{quote}
    ``...If I were to get hacked or the person [I share it with were], or if the organization storing it...[were] to get hacked, then my content would be leaked 
   % all over like, the internet, 
    and that's the main reason I haven't thought of [storing] it online." 
\end{quote}
% Alternate quote: I prefer stuff to not be connected to the internet and then I just like trust it a little bit more. P31
% Additional quote from C44
%Others continued to use cloud/file share platforms but disabled automatic backups.
% to prevent intimate content from leaving their devices. 
%Using a hidden folder was another common strategy, which we elaborate on in Section \ref{subsect:storage-strategies}.

% Those who used external hard drive mostly did so as a supplemental storage method for backing up intimate content. 

% \subsection{Threats}
% \label{subsect:storage-threats}
% Regardless of the storage mechanism selected, almost two-thirds of participants explicitly reported at least one of the following concerns.

% \smallskip
% \noindent\textbf{Hacking.}
% % P: 5, 8, 9, 11, 12, 14, 16, 17, 19, 22, 23, 26, 30, 34, 35, 38, 45, 55, 56 
% % count: 19
% % Viruses, phishing
% Although many described hacking as, 
% % ``more of 
% ``a hypothetical background fear" (P11), more than a third of participants were concerned about it as a means of accessing their intimate content.
% % forms of storage being hacked. 
% They brought up viruses, phishing scams, and malware such as, ``a virus that can be installed on my computer and have access to my photos and folders" (R8).
% Many others, however, viewed hacking as an individual, targeted attack and felt this may not affect them.%, though,
% % Our participants varied greatly in their concerns regarding hacking. Many had evaluated the likelihood of being personally targeted and
% %decided that 
% % their personal situation did not warrant consideration of this risk.
% For example, R21 explained,
% %this hack situation is very tricky, because who wants to hack you? I mean, that's the first question. 
% % ``If nobody wants to hack you, 
% ``because you're not important or because you're not [on their radar] why you are going to be worried? %But for the meantime, I'm not worried about to be hacked, for example. But yes. It would be... 
% I would be worried if I started to get into a position that feel[s like] I'm a person that someone wants...to hack."


 \subsection{Safety Strategies}
 \label{subsect:storage-strategies}
At least two-thirds of participants explicitly took one step to protect their stored content.
% \textbf{Disabling automatic backups.} \lucy{TODO}

\smallskip
\noindent\textbf{Deletion.}
% P: 2,6,7,8,9,10,12,13,14,15,17,18,19,23,27,31,33,34,35,43,45,46,48,49,50,51
% \elissa{be consistent in giving prevalence -- about a quarter, half, whatever -- in all these strategy sections throughout the paper or nowhere; time permitting it would be nice to have everywhere so the reader realizes people are really being intentional; you have in the two sections below but not this one}
% \lucy{there were also interesting quotes about deleting bc ppl didn't like the image over time or bc of storage but those didn't feel like mitigation strategies so i didn't include those. quotes are in comments tho}
% One technique participants practiced 
Around half of our participants proactively deleted their content
% engaged in proactive deletion of their content %Some participants chose to routinely delete intimate content from their storage methods primarily 
to reduce 
% risks associated with hacking, device theft, or accidental content reveal to unintended recipients/viewers.
the risk of discussed threats such as R14,
``İ usually delete videos or very explicit photos because I prefer not to keep them on my phone in case someone steals it."
% was deleting content they had created of themselves. 
% Multiple participants shared with us that they deleted content out of the fear that others would accidentally see it. 
%Specifically, P22 and P31 mentioned that others, such as family member or friends, may use their devices or want to view their phone's photo gallery. 
% They therefore deleted intimate content from their devices to prevent others from accidentally finding intimate content. 
% For example, 
%P10 additionally highlighted the fear of accidentally sharing intimate content when sending unrelated pictures, due to it being in their phone's photo gallery. 
 % Or like sometimes on my phone, I'll go through my images, folders. And just sort of try and take all the nude content out. Just in case someone wants to like, look at your photos on your phone, but I don't do that super regularly or something.  (P31, Pos. 73)
% Accidental discovery: P22, 
% The primary reason is I fear of being exposed
% 19:21:06 P
% 	when I'm home, my little cousins (one is girl, 9 yo, and other one is boy, 4 yo) always use my phone and check my gallery
%  (P22, Pos. 26-29)
% Honestly, I delete them pretty fast, just because there's always that anxiety. 'Oh, God, what if I accidentally send', I'm trying to send one image to a friend that actually sent this one I'm probably going to leave that instead. [...]  It's like, I have too much of an anxious brain and I'm like, I gotta go and I gotta go and delete that image because I can't otherwise. (P10, Pos. 170-175)
% Yes. I think from... not sure about mine, never, don't remember. I mean, when I change the phone, I just before... because all my old phones I give to my relatives, so just like delete everything, clean it completely, and that's it. As for the received intimate content, it's in the histories of conversation. So there I only deleted it once as far as I remember, because of like, emotional reasons, but that's it. (P7, Pos. 32)
% Others (P14, P34, P38, P45) textbfasized concerns that someone could discover their intimate content if their device was stolen or if their method for storing intimate content were to be hacked.  
% I was aware of the risks of keeping sensitive content on my device + I heard many things about revenge porn, hacking devices and stuff like that 
% one of my priority is safety (P34, Pos. 34)
% I actually don't feel very comfortable having the content in my phone, in case it gets stolen or hacked or, I don't know. But then I know that also, whatever I shared already, is out there in the world. I have no power over it. (P45, Pos. 137)
% Ah, not too often. If I if I go back at something, and I'm like, Ooh, you know, because I think I'm like always aware that like, if someone takes it, if someone steals it, is this what I want in the world? That's like, you know, if I look really hot in a picture, well, yes, it's fine, yeah, enjoy. (P38, Pos. 45)
% P  20:50  
% As in what I was mentioning earlier, that my phone might be hacked or someone could...? 
% I  20:57  
% Yeah, I guess so. 
% P  20:59  
% Yeah, I'm always having this in mind. And I'm scared...
% I  21:04  
% ...theft and hacking? 
% P  21:06  
% Yeah, exactly.
% I  21:07  
% Are there any strategies that you use to mitigate these risks?
% P  21:12  
% Just by deleting the pictures every now and then, actually. (P45, Pos. 280-293)
% P:  İ usually delete videos or very explicit photos because I prefer not to keep them on my phone in case someone steals it. The other « nude » content is usually without my face so it’s not relevant (P14, Pos. 16)
%\lucy{More structured vs. haphazard}
% Their deletion practices 
This included: deleting from a device after transferring to more secure storage (C34), deleting only photos with intimate body parts exposed vs. ``lewd'' images
% that were intimate by implication 
(R18), 
% deleting when they have changed their appearance in some way (P12), 
deleting from cloud storage after automatic backups
% was enabled for other photos 
(R17, R23), regularly deleting content after some period of time (C24, C41) or when they happen to come across intimate content in their photo galleries (C46) or when surfaced by a ``memory'' feature (R6, R45):
\begin{quote}
``...if my [\textit{cloud storage}] will send me like, memories of [intimate content] %or something. [...] 
% I'm just like, trying to sip my tea and have a relaxing day and I'm like... 
% Yeah, 
%sometimes when my like, nudes or whatever, get mixed in with just my normal photos. 
That's where I'll be like, yeah, get out of here." (R45)
\end{quote}
% Deletion patterns: 
% I would say I always delete the videos after few weeks/one month maximum; and for the pics I keep the ones that I think are more artistic or where I like my body the most (P24, Pos. 63)

% Um, that's a good question. Maybe when I remember I have something I would not like to be seen on my camera roll. Yeah. (P45, Pos. 141)
% CLOUD
% I have. But usually, when I see that intimate stuff has also gone to the cloud, I usually delete it. (P23, Pos. 12)
% then I delete everything stored on my device, it is stored on a kind of cloud (P34, Pos. 30) (after transferring to am ore secure storage location)

 % don't think so. I think, well, actually, maybe I have, I think I used to, you know, when I was using email to share things, I think I was storing things on the cloud. But then, you know, I realised that maybe that wasn't as secure as I hoped it was. So I deleted the things I was storing on the cloud.  (P29, Pos. 108)
% I mentioned since I've automatically started backup my photos to Google Photos, I delete them from there now. (P17, Pos. 153)

 % So, you know, if I got real new hair, or if there's something like that, then I will clear out the old ones because especially older ones, like I guess they're not like they're for me in that I get something out of sending them.  (P12, Pos. 25)

% What do I do? Nothing like, structured. Imagine how a lot of the time a lot of time probably delete it quite quickly after, a momentary purpose. Other times you may be used as a like you can hide folder, right when I when iPhotos. So I guess I'd rather than delete it, I'd probably hide. Yeah. And I would delete it quickly occasionally hide it. Yeah, I don't recall, particularly periodically going back and delete and (P6, Pos. 45)

% I think I store more than I used to. I think that I used to go through and delete things more often. You know, because I think that I was a bit more worried about it to a certain extent. But now that I kind of feel more secure in those things, like I don't, I kind of, like delete them as and when now I suppose being like, I think that often times, if I sent them, I would very quickly delete them in the past, whereas now I'm just sort of like, you know, we'll get to it when I get to it. You know, when I'm doing a generalised photo cleanup. Yeah.  (P12, Pos. 157)
% Yes I delete content sometimes, mostly because I don't like it anymore and don't plan to use it again, I used to check what I keep like one time a year and delete what I don't like (P41, Pos. 20)

% Yeah, so I don't usually take pictures of my genitals, like my vagina and vulva. And I think that because I do struggle with a bit more shame about these kinds of images that I often delete them. Yes, so there's certain images that I really like keeping such as full body or of like my breasts or my ass or whatever. I mean, there's non nude sexualized nudes that you can take well. But there's something about the... when like genitals are involved, it does make me feel a bit of shame and embarrassment that those are the kinds of images that I might feel uncomfortable if somebody were to find them on my phone. (P18, Pos. 104)
% I have other aspects of my life and I do not want to disclose this particular activity to other people: after a long photoshoot or a series of videos, I tend to move them out of my phone (P33, Pos. 59)



% Don't like image: P56, P47
% I don't like like it anymore, or it's something that I made, like, maybe six months ago, and I never used or uploaded it, then I just get rid of it. (P56, Pos. 196)

% Yes I delete content sometimes, mostly because I don't like it anymore and don't plan to use it again, I used to check what I keep like one time a year and delete what I don't like (P41, Pos. 20)

% o I think there's not really a timing to it, or like, I do it that often kind of situation. It's just, yeah, sometimes when I don't like an image anymore, for example, just like when I don't like the aesthetics of it, I will delete it, because I don't think it looks good anymore.  (P31, Pos. 73)

 % I guess if I'm just not comfortable with pictures I add, or if I take multiple pictures at a time I save one at the end. (P16, Pos. 36)

% Yeah, yeah, sometimes I delete things, or I have them in an old computer. And that's it. Old content that I don't like anymore. But most of it, I resell it, like old videos or old photos, I repost them, because a lot of times the users, the subscribers, doesn't realise if it's an old or new photo. So I recycled content. So I have most of my content in my phone. (P9, Pos. 28)

% Yeah, I think like, change of relationship would definitely cause me to do that. And yeah, like body image or something like that. Like, if I wasn't happy with the way I looked in certain images, I delete those, like, of myself, I delete those. And if anyone said that they wanted the images deleted it, I delete them as well. (P13, Pos. 37)

% And kind of like when I'm running out of storage or when something doesn't appeal to me anymore. I don't like certain images. Yeah. (P53, Pos. 120)

% I  3:28  
% Okay. And do you ever delete content?
% P  3:34 
% Yeah, if I hate it (laughter) if it doesn't work for me. Yeah.  (P38, Pos. 34-37)
% Um, well, not really like, what I do is I will delete some of the pictures from time to time if I don't like them anymore or not. Sometimes this keeps some of the pictures to send in, in certain situations, cause sometimes you're talking to someone and you don't feel horny, so you don't get hard. And so did you send something that you have already saved? But you have like any special routine? Just to take the picture? That picture was there.  (P3, Pos. 145)


% Sometimes I delete it when I don't like it. But sometimes I delete the pictures from my Twitter account and from my (inaudible) account, because I work also, I didn't say that sometimes I work as an escort. So sometimes I delete my content when I think I'm not safe, I mean, I sometimes I have evenings when I feel insecure. And I check which picture is maybe more, shows too much skin. And I don't want to show in public. In main account, I don't want to show some parts of my body. (P49, Pos. 52)
% Yes, I have to admit, I've totally deleted some pictures from (inaudible), from the second app that is mainly for my escorting things. Because first, it was bad for me when I sent my pictures to feel okay with my body, my sexuality, because I'm from a very Catholic household and country and I wasn't... for a long time in my life, I feel bad about my sexuality and my body. And it was platform to deal with that. But when... so yeah, I deleted a lot of, a lot. There was, I don't know, maybe eight pictures. And now I have two pictures on that platform where... and I'm completely, I'm in my clothes. So and, and there is yeah, I'm in my clothes, and I deleted more like naked pictures. And also I deleted some of Twitter pictures when I have, after that (inaudible) from last week. I deleted pictures when I wrote that my birthday is today or something like that. Or when I wrote that's, I didn't know... I when I wrote the name of the city I live, I deleted those. (P49, Pos. 160)

% Storage:
 % I guess I delete it if I don't like it. Either the backup or the original. And I might also delete it if I am running out of storage, mostly because most of these pictures with the exceptions of some that I might really like, because I don't know, they were very artistic or something, most of these you can take again, I think. So  it's not like content that I will be really sad if I lose. So I might delete it. Yeah. (P47, Pos. 40)

% And kind of like when I'm running out of storage or when something doesn't appeal to me anymore. I don't like certain images. Yeah. (P53, Pos. 120)

% But it's basically because of the, the amount of storage capacity I have, so I need to delete things. But it's only for that reason, you know. (P39, Pos. 60)

% Yes, I do delete stuff. And I sometimes do that, when I create some content that it's not, it's not up to a standard that I have meant to. So after creating something, I might see it again and dislike it, then I might delete it. I sometimes also delete big files, just for storage, saving some storage. (P37, Pos. 37)

 % it's a limited harddrive on the phone. So at one point, you have to delete something. (P51, Pos. 132)

% Random: P43
% It's less regular, it's pretty random. Just you know, sometimes you feel like you have... sometimes you go through your photos and be like, Oh, I have this and this. I don't want to have it any more and then you will delete it. (P43, Pos. 100)
\smallskip
\noindent\textbf{Authentication.}
% P: 7, 8, 12, 28, 29, 33, 42, 48, 51, 13, 29, 53, 
Participants mentioned password protection and authentication for general security but a quarter were intentionally mindful about these practices for intimate content.
% to prevent against threats.
% hacking, theft, and/or accidental discovery.
They  
% A few participants (6) explicitly mentioned
used strong passwords, biometric authentication, two-factor authentication,  password managers, and/or  password-protected or encrypted folders.
% for intimate content.
% Locked folders: 13, 8, 48, 51, 42
% A few participants (5) used password-protect folders to store their intimate content, such as C48, who shared a computer with their children p

\smallskip
\noindent\textbf{Hidden Folders.}
% Text from storage section:
% To prevent this several (12) participants including P46 used hidden folders on their mobile device %(P6, P4, P30, P46, P14, P16, P23, P54, P51, P29, P11, P2), 
% so that the potential to stumble on to nudes ``doesn't happen anymore because I just put a little private like thing on them so that they will go into like a secret folder or whatever'' (P46). 
% Hidden folders are not enough to prevent all risks of mobile storage, however.
A quarter of participants used a hidden folder, which excludes selected photos from a user's photo gallery and places them into a designated folder (e.g. Apple \cite{apple_hide_nodate}, Samsung\cite{samsung_what_nodate})
to prevent the unintentional discovery of intimate content.
% while others 
%strangers, etc.) 
% used their devices, shared cloud storage, and/or looked over their shoulder. 
For example, C46 commented that, 
``...sometimes when I'm just going through like, my regular day photos and like nudes will pop up, [now that I'm storing in a hidden folder] that doesn't happen anymore."

% \elissa{the password protected folder stuff down here should go in authentication in terms of the counts}
% because I just put a little private like thing on them so that they will go into like a secret folder or whatever." 
% The most common practice (P6, P4, P30, P46, P14, P16, P23, P54, P51, P29, P11, P2) was use of a hidden folder on a mobile device.
% For example, a few participants explicitly mentioned the hidden folder feature on iPhones that excludes selected photos from a user's photo gallery. 


% Lock folder (P34, P13)
% but tried to have it just on this hard drive where I also, I think I tried to password protect the folder, but I don't know if actually ever did.  (P31, Pos. 65)

% For me, for the one that I use the most is Google Drive. And I think the good part of Google Drive is that you can do very specific... like content protected with passwords that you can sell the password to access, things like that. To make it easy and more or less secure to... (P42, Pos. 234)

% it is called "KeepSafe", an app on which I can transfer medias on it, like a private vault, using a PIN code to unlock it and store content (P34, Pos. 29)

% Yeah. So I use, like Google Photos. So I guess that's cloud and an app. Yeah. And they have like, a locked folder within that.  (P13, Pos. 13)  And then I learned about that feature, and with the locked folder, and just found that really, really useful. (P13, Pos. 29)
% \lucy{Briefly mention points below elsewhere}
% On desktop computers or laptops, a few participants (R13, C48, R47) shared that they would nest folders within one another to hide intimate content or use password-protected folders. As C37 shared, "I've created a folder that's named `personal stuff`. Inside there, there are many, many, many more folders. So it's actually hidden inside another folder..." Another tactic, used by R47 and C37 was to deliberately name a folder containing intimate content something that would deter others from opening it. R47 chose a more obscure name,
% "I am a little bit paranoid about it having, you know, a very descriptive name, obviously, 
% "...I'm not going to write something like, nude pictures of me on the title [of the folder]. So I usually put something like, neutral, or something that is nonsensical. [...] So something weird, like a weird phrase, or something like that is what I do." Meanwhile, C37 added that they explicitly labeled a folder "porn" so that others would assume its solely for their consumption and not open the folder.

 % So it's actually hidden inside another folder, that's called "personal" and then there is another folder that's called "porn". So I'm I'm hoping that if someone sees a folder that's named porn, they will assume that is porn for my consumption and will not bother to open it. (P37, Pos. 21)

% "So yeah, they'd probably be like hidden in some, like, you know, off the grid folder like that no one would stumble across. Like not named something that you know, is obvious, but that's not very secure. Or like yeah, I don't know, like a locked folder or something like that. But yeah, I didn't really have much worry of someone like getting into it. " P13


% "So I use, like Google Photos. So I guess that's cloud and an app. Yeah. And they have like, a locked folder within that [...] I started using like cloud backups for other kind of documents and personal things, because I was running out of physical space. And then I learned about that feature, and with the locked folder, and just found that really, really useful." P13

% then I started organizing a little, with folders on my computer (some I locked just in case, I have children)
 % (P48, Pos. 38-39)

%  And WhatsApp, I have my own folder where I keep them, which is kind of separate from the other folders, again, to stop the scrolling issues when you're looking for a folder amongst your friends and one pops up. Actually, mind you that's happened to me with several of my other friends in the other direction. I've caught a glimpse of their nudes, let's say, so that's not the end of the world either, I suppose. Yeah. Other than that, that would have been the main ones. (P17, Pos. 153)
 
%  "I have a private folder. So like for, you know, I was talking about sometimes when I'm just going through like, my regular day photos and like nudes will pop up, that doesn't happen anymore because I just put a little private like thing on them so that they will go into like a secret folder or whatever. Just so that they're not quite as like obvious. They're definitely still there but yeah." P46


% Naming a folder something nondescript to avoid it from being noticed: 

% \begin{quote}
% "I am a little bit paranoid about it having, you know, a very descriptive name, obviously, I'm not going to write something like, nude pictures of me on the title. So I usually put something like, neutral, or something that is nonsensical. [...] So something weird, like a weird phrase, or something like that is what I do." P47
% \end{quote}
% Nesting folders: 


% \smallskip
% \noindent\textbf{Local Storage.} 
% \elissa{@Lucy move all of t his to the security heuristic decision stuff in the prior subsection; you can keep this header and have one sentence backward pointing to that section}
%\lucy{@Elissa, removed local storage bc it felt like having a sentence here was repetitive but can add in}
% P56 (doesn't use cloud)
% I store everything offline. P53

  % I just keep it on my you know, hard drive, not the cloud. (P43, Pos. 252)

% I prefer stuff to not be connected to the internet and then I just like trust it a little bit more. P31

  % Storing files offline. I just feel like it helps in the sense that I'm sure that it won't be hacked. Also, I won't have like, mad anxiety that maybe afford it (?) or just got into like afford to store it under like a different email or something like that. I'm sure that even if I store it in another email, I might forget the email. And I might not be able to get back the content or if maybe the folder were to disappear. I usually have like mad anxiety that maybe my files might get lost or even delete themselves. Or maybe someone might hack the platform and leak the content or just... Yeah. I think like something bad might happen to it if I were to like, store it online. That's with like most stuff. And yeah, I just, I prefer storing folders offline. Just for privacy, and I can have like a sense of control over it. In that I know that I can retrieve it anytime I want. P53
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% MISC QUOTES START %%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % have never liked been fond of storing it. Or just purchasing my storage space online. Mostly because I think that if I were to get hacked or the person, or if the organisation storing it, and having the driver to get hacked, then my content would be leaked all over like, the internet, and that's the main reason I haven't thought of doing it online. And also, with buying storage, I have thought of... I haven't quite come to terms with what platform I'd like to use, what platform I trust more. (P56, Pos. 273)


% I tend to... I mean, I try to generally avoid the big, like, the big corporate cloud storages, even though it's a bit impossible these days. For example, my photos, my videos in general, I don't back them up on my Google Cloud or whatever. However, I do sometimes back them up on my computer, but that's a bit... It's not very systematic. (P47, Pos. 12)

% Yes, I used to... Years ago, I used to use the cloud, because it was easier, you can share it across multiple devices and so on. But then No, I stopped. I do not use that. I don't use it in the cloud. It's all stored in my phone. Even though I know it's not 100\% safe, I just keep it on my you know, hard drive, not the cloud. (P43, Pos. 252)

% When I store content, I think the most risky things now for me, it's if people stole me, that is not that big of a problem because as I said before, I am pretty... I'm pretty accepting that. But I think the most problem is if I had something exclusively in one website and in some moment in the near future that website close. (P42, Pos. 166)


% I mean, it would be... I mean, I really appreciate like apps that have organisational characteristics, like folders, or etiquettes, or things like that. WhatsApp, of course, is not one of those. Actually, one thing that I don't like about WhatsApp more than I do, is that, like, sharing big amount of pictures is like really... is not that comfortable. And it's like the I say, pretty chaotic. That's why when I have to share like a lot of pictures or long videos, I prefer to use like Google Drive, because it just upload that and organise them into folders. And that's it. Like WhatsApp, it's more like sending just a couple of things, or, or short videos or GIFs, you know. (P39, Pos. 242)

% Because you can lose a phone, or your phone could die for any reasons. And I would like to have access to my data. And that's, like, a backup all of my data. So I just go along with it.  (P26, Pos. 32)

% So yeah. Yeah, for hosting, I usually go to Hasna, which is a travelling cloud provider that has a reputation for being somewhat trustworthy with data protection. And also the accessibility. Yeah. So yeah, okay, for storage I also trust my iPhone that does... that it is not that easy for attackers to install any software on it. And I trust its security system when I need to grant explicit permissions to apps. So just I know that the operating system is keeping private data private against any apps that aren't explicitly allowed. And for services. I know that signal's end to end encryption is really, really bad. Okay, really, really bad. But, yeah. I've added the bits into the protocol behind it.  (P26, Pos. 128)


% Well, I like to save photos of myself, because I like recording my life, and like, including intimate aspects of my life. And I like being able to look back through those memories. And also just seeing my body, seeing how my body changes over time. And I think it's really important to backup your data. Hence, the external hard drives. Because I don't want to lose information. Obviously, there are data protection and security measures that cannot be completely accounted for. If my house burned down, I would lose everything. But I don't know. Yeah, I just... like I like making backups of data. And maybe I'll never access it again, but I like knowing that I have it. (P18, Pos. 96)

% Not many ppl talked about how things are stored in-app
% The one I send in no way. So just it's somewhere in the phone, and somewhere in the histories of conversations, I guess. Telegram mostly I guess. As for the ones I received the same, but I guess at some point, I might have downloaded it just to sort, I guess is the best word would be. And in both of those cases, like nothing more than a folder, I guess. (P7, Pos. 12)



% I guess the only kind of fear I have in keeping them on my phone is that, you know, I'm scrolling through looking for a photo in front of someone else, they might kind of pop up essentially. Other than that, that's my only kind of concern with kind of storage place around there. But to answer your question mainly, just convenience,  it's stored there, because that's where I need it. (P17, Pos. 29)


% I mean, I think that just having an iPhone is like, a complete... It's like completely giving up on your privacy. Because if you... I don't know if you've ever tried it, but if you look for the word bra in your gallery, it's going to show all of your bra pictures. So yeah, I mean, yeah. (P23, Pos. 192)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% MISC QUOTES END %%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% removing from cloud %%%
% A cloud? No, I don't use the cloud for revealing photos. I do not, in my phone there's no... it's not attached to the cloud. I removed cloud services of keeping photos. (P43, Pos. 88)

% Convenience, I suppose, you know, I need them on my phone to send them I guess, so that's kind of it, really. And I back them up. Because I have the automatic backup on Google Photos. I don't do that on purpose. The fact as I said that I tried to delete them. But this is more convenient to leave it on really. (P17, Pos. 25)

% Okay, we can say that sometimes. If a photo is stored locally, there is a concern that it may be just uploaded automatically without my concern. For example, within iCloud,  (P8, Pos. 181)
% But I double check that, to be honest. So to be to be sure that it's not even in the trash of iCloud. But yes, there is always this concern if some time I forget that. Doesn't find that online in the cloud. (P8, Pos. 185)

% No, I never [store on a cloud platform]. I just like keep them because I like them. But just like my my photos, I never like download photos of everyone who could say send me some. And I wouldn't like to have them on cloud or just like, I wouldn't like them to be traceable. Or just like stored forever somewhere. I could not really access at any time. (P30, Pos. 13)

% Sometimes I've thought about it like, it's just like a thought that... Well, what if my cloud gets gets hacked? So I delete my pictures from the cloud. I don't really expect my PC to be hacked. I don't think it's gonna happen. (P23, Pos. 200)

% OLD TEXT
% Participants stored intimate content within the photo gallery of their mobile device, on a cloud platform, on a laptop or desktop computer, on a hard-drive, or within an app used for sharing intimate content. Sex worker participants in particular, tended to share larger files so they more often used hard-drives, laptop/computers, and cloud platforms.

% \lucy{Not all participants were comfortable storing intimate content... (add quotes about discomfort around storage)}


% \lucy{TODO: this was the first section I wrote and needs counts to be added. Will come back to this!}
 
 
%  \paragraph{Mobile Device} The most commonly used storage method among our participants was the photo gallery within their mobile device. Frequently, participants mentioned using a hidden folder within their photo gallery, which we discuss in more detail in Section \ref{strategies-technical}. Since participants are often creating content on their phones, images and videos naturally are stored within their photo galleries. For those who used their mobile devices to send content, having intimate content within their photo gallery was convenient for sharing the content. 

% %  "it’s slightly dangerous to keep your own intimate images on your phone, if I had a more secure solution id totally use it!" P14
 
% %  "I started it four years ago, I think, when I had my iPhone, because before I use the Snapchat and I kept them in Snapchat. But I didn't have them in my in my gallery photo. And now I don't use Snapchat anymore I just a.. So yeah, I think 2018. [...] Um, I think it was just my boyfriend who showed me how to hide some photos. Yeah, I think it was him who showed me it was possible." P30
 
 
%  Many individuals also supplemented their mobile storage with a backup option on a cloud platform, computer, or hard-drive, which P26 explained, "Because you can lose a phone, or your phone could die for any reasons. And I would like to have access to my data. And that's, like, a backup all of my data. So I just go along with it."

% \lucy{Could probably remove this quote...}

% % It's convenient. It's unconvenient when it gets stolen. And once my phone was stolen, containing a lot, a lot, a lot of personal images and data and... but luckily, it was an iPhone, and they have this option to delete and erase everything from, like, from a computer. So I was like, at one point, I mean, it was locked and everything, but I was like, Oh, my God. Oh, my God. P51


% \paragraph{Cloud} For both supplemental backup and as a primary storage option, various cloud providers (iCloud, Google Cloud/Drive/Photos, Dropbox, MEGA, Hasna) were used among participants. Participants commonly began using cloud storage as an automatic backup from their mobile device. However, some chose to manually back images and videos up on a periodic basis or when they remembered. When deciding to use a cloud storage option, convenience was a cited reason. Three participants (P35, P40, P16) explicitly mentioned that they valued how easy it was to access their content using their preferred cloud option, especially when accessing across multiple devices or accounts. Another reason participants (P35, P27, P13) chose to use cloud platforms was due to storage constraints, such as their mobile device running out of storage space. A few participants also used cloud platforms for sharing intimate content and therefore stored the content there for others to access. As P52 explained, "Sometimes, I also transfer the content to clients, if somebody would like to buy a video, but they don't want to go to manyvids. Then I upload it on Dropbox, and I share the link with them after the payment."

%  \lucy{Comment from Elissa: "wondering if we should use C\# and R\# to distinguish commercial \& recreational participants"}

% % - Convenience: Having things in one place (P35, P16), easier to access from anywhere (P40), user friendly/easy to use (P48, P45)



% % while others explicitly turned off automatic as a mitigation strategy to prevent intimate content from being backed up. P8 elaborated on this concern, "If a photo is stored locally, there is a concern that it may be just uploaded automatically without my concern. For example, within iCloud."
% % \lucy{I feel like it was supposed to say consent and not concern}

% % - Heavy files or needing additional storage (P27, P12, P13) 

% % -Also how they share 

% Participants also mentioned using cloud platforms for storing other types of files but explicitly preferred not to have intimate content stored on a cloud. As P17 shared, ``But the fact that my intimate images can be on the cloud really makes me uncomfortable. Because it feels like it's somebody else's property." To prevent intimate content from being uploaded to a cloud platform, participants mentioned turning off automatic backups or manually deleting intimate content, which we discuss in more detail in Section \ref{strategies-technical}.

% % For participants that 
% % \begin{quote}
% %  Well, I guess yeah, there's a risk of like the cloud, I think. [...] Then again, it's just like it's way more accessible, but also has so many consequences. 
% % \end{quote}



% % - Explicilty do not want cloud to auto backup: (P17, P23, P33)
% % "Because I have the automatic backup on Google Photos. I don't do that on purpose. The fact as I said that I tried to delete them. But this is more convenient to leave it on really. [...] " P17

% % "when I see that intimate stuff has also gone to the cloud, I usually delete it." P23

% % "all my pictures were stored on my phone only and now, they are on the cloud, which I do not like at all (P33, Pos. 180)"



% % - Ppl storing other things on cloud already (P12, P13)
% % started using like Cloud backups for other kind of documents and personal things, because I was running out of physical space. And then I learned about that feature, and with the locked folder, and just found that really, really useful. P13
% % I've just kind of got like a photo archive that I that I keep on there, and it'll have all sorts of things. But it will also have, you know, sex things on there, for sure. P12



% % One participant noted that they had switched from hard-drive to cloud specifically for the convenience. 

% % Google Photos, it's automatic. I don't have to do anything. Super nice. My camera roll. So that's mainly why I use it. And yeah, yeah, just so convenience. And it's already integrated with the rest of my Google account, so everything is in one place. P16
 

 
% %  "My storage has gone from less harddrive... Not on, like so much on my external hard drive anymore. More cloud based. But also, I don't, if I like was to make the conscious decision to like not make it cloud based I think it wouldn't be too much of a problem, because I have a really fucking, like, high storage on my devices these days. Like, it's not as important to be using Cloud Storage for me now. "

% % - manual backups (P12
% % No, I periodically do it. Yeah, I don't do an auto backup. I don't know why I don't do an auto backup. I probably should, because it would encourage me to delete things more often when my phone is really full. But yeah, I just kind of like do it every, you know, few months or so. Like six months or so I'll be like, 'Oh, this is getting full. I'll, I will back everything up'. Yeah. P12
 
% % User customized storage solutions:
% % "I regularly transfer all the images from my Android phone to my laptop. And I also make regular backups of all the data on my laptop on an external hard drive, that I do not encrypt any of the pictures." P18
% % [nesting folders quote--need to find]


% % "So whenever I have intimate photo of myself, I put it on a Google Drive. But I don't leave it on my phone. I mean, it's in the app. So in Grindr, and in Google Drive." P4



% % Convenience may mean different thing sto different people

% % "So in Google Drive, no, I don't really like Google Drive to store pictures. Because it's pretty hard to see the miniature. You know, when you want to have an overview of all the pictures, at the same time, it takes a lot of time to charge. And so when I'm looking for a picture quickly, it's not convenient." P4

% \paragraph{Laptop/Computer} Multiple participants used a laptop or computer to store intimate content with the main reason being the need for more storage. Additionally, one participant commented on the convenience of having content stored on the same device they use for editing. Participants also chose to use their laptop or computer to back up intimate content. Two people specifically noted that they had security concerns surrounding cloud options and preferred a more physical option. For example, P56 shared, 

% \begin{quote}
%     ``...I think that if I were to get hacked or the person, or if the organisation storing it, and having the driver to get hacked, then my content would be leaked all over like, the internet, and that's the main reason I haven't thought of doing it online." 
 
% \end{quote}


% % - Lack of storage on phone + fear of losing content (P53)
% % - Better storage + editing is done on laptop (P56)
% % - lack of trust of big platforms 
% % - backup (P47)
% % - 
% % "I tend to... I mean, I try to generally avoid the big, like, the big corporate cloud storages, even though it's a bit impossible these days. For example, my photos, my videos in general, I don't back them up on my Google Cloud or whatever. However, I do sometimes back them up on my computer, but that's a bit... It's not very systematic." P47

% % - concerns about device sharing (P37)
% % - concerns about hacking

% % P56 expressed that they prefer to use their laptop because of security concerns with cloud options. "I have never liked been fond of storing it. Or just purchasing my storage space online. Mostly because I think that if I were to get hacked or the person, or if the organisation storing it, and having the driver to get hacked, then my content would be leaked all over like, the internet, and that's the main reason I haven't thought of doing it online." (P56)
 



% \paragraph{Hard-Drive} Some participants chose to store intimate content on an external hard-drive.  Among them, most used an external hard drive as a supplemental storage method for backing up intimate content. Some also mentioned that this was their default supplemental approach for backing up other types of files as well. 
% \begin{quote}
%     ``I like to save photos of myself, because I like recording my life, and like, including intimate aspects of my life. And I like being able to look back through those memories. And also just seeing my body, seeing how my body changes over time. And I think it's really important to backup your data. Hence, the external hard drives. Because I don't want to lose information." (P18)
% \end{quote}

% Another reason participants chose to use an external hard drive was due to security and concerns surrounding hacking or others accidentally viewing intimate content on their mobile device or computer. As P44 explained, "I have this hard drive so if someone goes to my computer, then they are not gonna find it by mistake or something."

%  Despite some  security concerns being alleviated by using an external hard drive,  others expressed that there are still risks with storing content on an external hard drive such as the hard drive being stolen or breaking. P41 shared, ``The risks I consider the most is more like if someone steal my hard drive, or if I lose it, when I'm on the go for example."


% This method, however, was not necessarily the most convenient for some participants who expressed that they have since switched to backing content up on a cloud platform or added a cloud platform to their backup process in order to more easily retrieve files.


% % - Keeping a copy (P27, P18)
% % - Already using for other purposes, general photos, etc. (P18, P31)
% % -Using only for larger content files (P50)
% % -Periodic backups
% % -P4 concerns about hard-drive breaking
% % - concerns about stealing (P27)
% % - mention of additional security, password, etc (P27, 53, P18)
% % - storing w/o additional measures (P53)
% % - switching from hard-drive to cloud or adding cloud (P52)
% % - Concerns of hacking

% % "And I got more cautious with even my drive, is that everything has a passcode. And yeah, I'm definitely the only one who can like open my folders up and my devices up." P53

% % Others mentioned that it seemed odd to 




==> strategies.tex <==
\section{Safety Maze: How People Try to Defend}
\label{sec:strategies}
Despite concerns, participants did not want the threats previously described 
% in the prior section 
to stop them from exercising their rights to sexual expression: ``I don't want to allow shame or stigma to prevent me from living my life and exploring my sexuality as much as I want'' (P18). As a result, all adopted strategies on both an interpersonal and content level. Many were optimistic about their ability to handle
% ---emotionally or via their specific strategies---
the potential consequences they may face if these threats became reality. 
%
%\lucy{@Elissa, Changed subheaders to include removing identifying features + watermarking into "content-based" bc it felt like they made sense grouped together w/ the stuff that was prev in "technology-based"}

\subsection{Interpersonal Strategies}
\label{subsect:interpersonal:strategies}
People applied strategies at the interpersonal level that related to how they navigate trust with recipients.
% such as rule setting, trust heuristics, consent checking and screening/vetting to protect themselves. 

% Navigating the landscape of trust and boundaries was a nuanced issue. Participants ranged in their expectations of privacy and sharing of intimate images.
% \lucy{@Sharon}
% \lucy{talk about explicit + implicit, hierarchies of trust, established relationship only}
%
%% themes:
% explicitly asking consent of recipient - P2 P17 P21 P23 P29
% assess the vibe - P2 P3 P6 
% instruction to open later/content warning - P26 P43
% of legal age - P3 
% assume always welcome - P30
% implicit understanding/trust to not share - P2 P3 P5 P6 P7 P10 P15 P22 P26 P28 P29 P31 P33 P40 P41 P51 P32
% explicitly asking to not share - P11 P12 P23 P33 P34 P35 P42 P43 P44 P45 P1 P20
    % certain situations - P4 P7 P14 P26 P51
    % explicit rules/expectations or boundaries - P6 P8 P12 P13 P17 P22 P26 P30 P37 P39 P47 P55 P20
    % permission to share - P12 P26 P20
% hierarchies of trust (more comfortable taking risks with trusted people) - P4 P5 P6 P7 P8 P12 P14 P16 P22 P23 P24 P26 P28 P29 P30 P35 P41 P43 P47 P48 P1
    % at first but then not later - P22 P33 P41
    % in personal life but not SW - P24 P46
    % in personal life and SW - P34
    % depends on the app safety - P17 P23 P24
    % payment - P33 P38
    % no obligation to reciprocate w/ nude - P7 P13
    % reciprocity = trust - P4 P5 P6 
% established relationship only - P2 P4 P6 P7 P9 P10 P11 P18 P19 P29 P30 P33 P35 P44 P52 
% do NOT explicitly ask to not share - P3 P4 P6 P8 P9* P15 P18 P19 P24 P27 P28 P29 P37 P38 P39 P50* P52
% threaten consequences - P30 P31 P34 P38 P47 P1
% don't mind if shared - P3 P4 P5 
%
\smallskip
\noindent\textbf{Rule Setting.}
About half of participants held the implicit expectation that their intimate content would be kept private and did not have explicit discussions with recipients around sharing it, especially among those who shared content with their established relationship partner(s) (see Section~\ref{sec:use:case}). %P6 expressed, ``I suppose like I feel as like a code of conduct, even though it's not explicitly written...[in] the communities I would interact with.'' 
When sharing with friends, P31 explained, ``trust was so established that it didn't feel like you needed to say [explicitly].'' 

The other half of participants explicitly asked recipients not to share or store intimate content. ``...I asked them not to screenshot anything, just to [keep] it in chat. And that was kind of the ground rule'' (P11). Sex workers in particular were more likely to set explicit rules. P35 shared: ``before I send images, I always just say that this image is between myself and yourself, and you're paying for this service. No one else is paying for this except you.'' 
% So this, hopefully will just be used by you. I say stuff like that." 
Recreational sexters mentioned that they would circumstantially ask for content not to be shared such as if they had friends in common (P4) or if there were identifying features in the content (P14). 
% P4, P7, P14, P26, and P51 
% mentioned they would explicitly ask in specific situations, if they had friends in common (P4) or if there were identifying features in the content (P14). 
% While other participants did not explicitly tell recipients to not share the content with others, 
%Many (13) alluded to other rules or expectations such as whom recipients were permitted to show this content to.
% and whether the recipient could save the content to their personal device. 

In addition, a few participants stated direct consequences if content were to be shared. % Another tactic participants utilized% to strengthen the privacy of their intimate content % was to threaten consequences.
For instance, P30 said, 
% ``Like before sending 
``I would just tell them, if you ever shared, I will come up to you, we will go to the police'' whereas P34 sent reminders to clients about potential consequences:
% ``it is clearly stated in the [User-Generated Content Clause] of the platform [and] 
% ``I do reminders every time [...] Plus, 
``I send them the penal law articles regarding sharing/publishing porn content.''

On the other hand, a few participants were open to recipients sharing intimate content if the recipients asked permission first or in specific contexts: ``I have on occasion, given people permission to share it with other people, especially in the context of [initiating group sex]'' (P12).
% you know, people that I'm having sex with being like, introducing me to other people [we might have group sex with]."
% or saying, you know, like, Oh, here's the, you know, especially this was in context where it'll, you know, like, group sex probably going to be a thing 
% [...] where it's like, oh, here's this person, he or she might want to also have sex with us, would you mind? And then I usually say, Yes." 
% \lucy{Should we mention the ppl who allow others to share here? Or somewhere else (maybe in concerns about IIA. I wonder if they change the content they send if they're allowing ppl to share??)}
% and three others sent content that they permitted others to share without asking permission.
% P12, P26, and P20 were open to their recipients sharing the intimate content with others so long as the recipients asked permission first while P3, P4, and P5 did not mind if recipients shared the intimate content without asking permission.

\smallskip
\noindent\textbf{Establishing Trust.}
Almost half of participants 
% (count: 21) 
expressed that they decided what to share (or if they shared) and their safety strategies based on their familiarity with a recipient: 
% had constructed hierarchies of trust in their head and were more willing to take risks with those they trusted:
%"So I have kind of, like, I guess, hierarchies of how much I trust a person, right? 
%So if I'm initially seeing someone and I'm like maybe they could do something nefarious with this, I'll never show them and send them anything that involves my head" (P12). Additionally P29 commented that,
% P29 added,
% \begin{quote}
    % "Who to share it with... So that would generally only be
% "people that I have already had sexual contact with. And it tends to only be people that I trust a lot. So that would be important to me. 
% So if, you know, 
% "say that 
% \begin{quote}
% ``[At the] beginning a relationship
``With somebody new, I wouldn't necessarily send them something sexy until we've been on a couple of dates, until we've had some sexual contact, until I knew that we were on the same page about privacy'' (P29). 
% \end{quote}
Participants may also regulate how explicit an image is based on their level of trust, ``if I am sharing with a person that I didn't fully trust, or think my relationship might change in the future, I definitely won't send them something as explicit'' (P13).
% And I don't tend to send very explicit, like content is just more like, I don't know. Like, semi nudity, or whatever. (P13, Pos. 125)
% \end{quote}
% Other participants shared similar 
% P47 added,
% \begin{quote}
    % "I guess that I have criteria, and I definitely do. They're not that easy, I think, to explain, I don't think they're completely explicit. They're a bit implicit. But at the same time, yeah, they're there. So I would definitely share it with a person I'm in a relationship with, I wouldn't have a problem doing that at all, I wouldn't even think twice about it. The criteria then have more to do with the people that I don't know very well. Or that I'm just meeting. I would choose to share, definitely, with someone that has shared first, I kind of feel that if someone has also shared content of themselves, it kind of makes me feel better to also share something of my own. So that could be a criteria sometimes."
% \end{quote}
Others had a more binary hierarchy and only shared within the context of an established relationship, such as P9 who shared content ``with a partner or person that I trust 100\%. [...] So if they will be leaked, I will know who were the person that put it out.''

% \lucy{Even tho section is already very lengthy, I think it's missing stuff about ppl who send in established relationships only}
% \elissa{this should go in hierarchy}

\smallskip
\noindent\textbf{Screening/Vetting.}
Vetting a potential recipient of intimate material was described by over a third of 
% both recreational and commercial 
participants who described speaking to recipients for some period of time prior to sharing content to assess whether they felt safe:
% \begin{quote}
    % "I'm starting to be afraid that somebody can do something like that [share intimate content nonconsensually]. And that's why 
    ``I'm really patient with choosing my clients. And I have to talk with them a lot to be sure that we can meet and nothing bad will happen'' (P32).
% \end{quote}
 A few participants relied on their intuition even without a conversation, such as P51 who shared intimate images through a dating app and described developing 
% participant using a popular gay dating app described having 
% ``developed 
``a sixth sense'' that they used to ``make a judgement based on various features on the profiles'' 
to establish if the recipient 
% was genuine and 
would be unlikely to re-share content.
% without consent.
Many sex workers relied on payment for screening. If the worker had payment details, they could take them to be
an implicit understanding that the content was for private use only. 
% e
% If a client had paid, the worker had some formal exchange or payment details from them and took this to be an implicit understanding that the content was for private use only.  %\elissa{@Vaughn check this phrasing} \lucy{Vaughn originally wrote this sentence}
% took this to be a type of contract that the client would be consider the content for private use only.
% As P9 described, ``I want to think that if someone is my fan, they're not gonna put these videos online.''
% \lucy{@Vaughn removed sentence about ID checks bc was a recreational participants who has been over quoted. Is there another quote that would be a good fit?}
% Sex workers also performed ID checks to make sure they were not distributing pornographic images to minors, ``the first thing to check is if they are of age''(P3).
%Recreational participants described similar processes, 
% ``I'm kind of trying to determine if I feel like someone is sketchy, you know, a very technical term there. (P12)''
%such as P51 who shared intimate images with others through a dating app and
% participant using a popular gay dating app described having 
%``developed a sixth sense'' that they used to ``make a judgement based on various features on the profiles'' 
%and establish that the recipient was genuine and would be unlikely to share the images non-consensually. 
%\lucy{Thinking about below and how does this differ from establishing trust...I need to think about more. Maybe establishing trust + screening/vetting need to be segmented differently.}
%
% Another participant added extra screening prior to sending images if they felt unsure of the person, ``I will ask the person to identify themselves by sharing with me their Instagram profile, or by having a quick quick video chat with me.'' (P4)


\smallskip \noindent \textbf{Deletion Request.}
Although in some contexts participants consented to their recipients storing their intimate content, almost a third had made an explicit deletion request. This commonly occurred after a breakup. Sex working participants made these requests in their personal lives and with clients. With their clients, P20 shared that this occurred ``when I sent them something that I later reconsidered... And it's usually when someone requests you to send them something on their DMS, some things that I'm not comfortable with sharing.'' However, P1 pointed out that this may be difficult after a transaction is completed, ``I even offered to like refund but no, [the client] didn't [delete the content].''
Across contexts, participants expressed that they were unsure if content was ultimately deleted. For example, P50 described an ``emotionally charged'' period where they weren't sure if their former partner had deleted their intimate images.

\smallskip
\noindent\textbf{Consent.}
%\lucy{Not sure that this is the right thing to name this}
%\lucy{@Elissa currently this is framed as consent bc this was previously named consent checking but maybe we should reframe.}
% ACTIVELY DO: P6, 29, 43, 12
Many participants mentioned the importance of establishing consent prior to sharing intimate content with a particular recipient but a few (4) mentioned in-the-moment consent checks, which they used specifically to check that a recipient is alone to prevent shoulder surfing, ``I'll always ask first and wait for their response before I send something because you never know what people are doing'' (P29).
% that there is a chance that they're not alone, I do send a note like, Hey, don't open it now, open it later. P43

% Participants also mentioned consent in deciding when to send intimate content. Some participants (P17, P21, P23, P29) specifically mentioned asking consent of recipients before sending content, while others (P2, P3, P6) assessed for implicit conversational and/or situational cues. \elissa{Like what?} P26 and P43 added additional instructions to open the content later in private.
% \lucy{Is this to prevent shoulder surfing?}

%\textbf{Resignation.}
%\lucy{@Vaughn} 
%\lucy{@Elissa we talked about potentially moving this to discussion. However, maybe we should split this up into feelings of resignation (to move to discussion) and some sort of strategy (which would stay in this section) where ppl only shared what they felt comfortable w/ other people discovering/being public}








\subsection{Content-Based Strategies}
\label{subsect:safety-technical}
In this section we summarize content-level mitigation strategies participants commonly mentioned.
% screenshot notifications, expiring messages, end-to-end encryption, metadata removal, removing identifying features, and watermarking. 
% For strategies that involve using specific features on platforms, aside from those who chose to use a platform based on the availability of a specific feature, most individuals used what they were able to find. 
Though less often described, participants also made use of features that enabled them to share masked content (e.g., recipients receive a blurred message and must click on the content to deblur it) and/or prevent the auto-downloading of images. 
%\elissa{@Lucy/@Elissa TODO: check that this list covers everything in this section}
%\lucy{Ended up moving unsending to its own thing bc there were more comments. Need to look again to see if there's anything else we missed in this list}


%\lucy{@Elissa I want to say something like this: "

\label{strategies-technical}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% expiring messages %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\smallskip
\noindent\textbf{Expiring Messages.}
% \lucy{todo: add more pro comments/reasons}
% % PRO:
% Actively use (56, as an option (29)
% Control over data (56)
% It's important for like, it gives me control over like the time and the person I'm sharing the content with. (P20, Pos. 313)
% I think is an is a quite nice feature, quite useful. Which I would like to see implemented in more apps, rather than only the more privacy focused ones.  (P47, Pos. 220) % DOES NOT USE CURRENTLY
% Yes, when they start doing this one time view, I'm all the time using it. And I also noticed that sometimes even if I'm sending normal photos of me, I still use it.
%  (P43, Pos. 260)
% so basically, as my account is free, I can only send one expiring picture a day, I do it sometimes when I really believe that the person I'm talking to is, is fake, or has bad intentions. [...] So yeah, when I go back to Morocco, I only use this, I only send expiring pictures... [...] So yeah, when I go to Morocco, which is a more dangerous place for homosexuals, I use this expiring pic feature. (P4, Pos. 201) % ALSO has a quote saying that he doesn't like this 
% I think it creates, yeah, this like more.. It it's kind of, yeah, it kind of replicates this thing that happen on like Adultwork and stuff where they can view that you choose how long the client can see the work if it's like four or five days, seven days a fortnight or whatever, that you can produce the same thing on there expiring messages as as well which is quite reassuring. Again, they can still save  (P35, Pos. 229)
% I think it'd be good to have the option to do that. Yeah, definitely. But not as a default. Because, you know, sometimes you want to go back to things later. (P29, Pos. 180)
% Oh, yes. Mainly for fun. Like, I think this is like, it gives kind of variation in terms of how the images can be distributed, which is nice for... in terms of like advertising and being able to send like teasers and stuff like that. (P46, Pos. 222)
% But if it's a stranger then, for example, yeah, you can delete messages on Grindr, which is nice. But then again, I also wouldn't immediately give my Instagram to a stranger that I've just met online. And, yeah, with Instagram, it's nice that it disappears. (P5, Pos. 233)
% I think that depends on the level of trust, but usually, I will just send them like on WhatsApp, like the nudes, and then in case I think that I have like overflown the other person with my pictures or the the amount of pictures are like a lot of them, I will start using the option of these pictures that disappear after you see them once. (P23, Pos. 24)
Expiring messages allow a sender to set a message expiration time. 
% after which a recipient can no longer view it. 
Expiration does not guarantee that a platform has deleted the content nor does it prevent a recipient from storing the content before expiration. This feature was widely used by three-fifths of participants (particularly recreational participants).
% . It was especially popular with recreational participants, over three-quarters of whom used the feature at least some of the time. 
Many used it situationally with strangers or in higher-risk contexts: ``when I go to [\textit{country}], which is a more dangerous place for homosexuals, I use this expiring pic feature'' (P4). Others used the feature to share more explicit content and implicitly communicate boundaries:
% it helped them decide on the sensitivity of the images, ``if the image disappears, I can be more explicit'' (P14). 
% Additionally, they were used to implicitly communicate boundaries,
``it’s a clear, unambiguous sort of caption that says I would prefer if you didn't hold on to this'' (P2). Participants were often aware that 
% Even for those who used it, they were aware that %In the midst of various concerns, many used the feature with the awareness that  
% Although some felt that expiring messages provided more control on when messages can be viewed, others who used them (P2, P18, P13, P35) 
 recipients could screen record, capture content with another device, or
% % This sentiment was captured by P2,
% \begin{quote}
% ``I think it's not fail-safe, because once the data is on someone's device, they will have any number of ways of storing it. So expiring messages is insecure by definition, almost. But I think the presence of it is reassuring to people. And I think it also... if you send someone a expiring message it's a clear, unambiguous sort of caption to it that says I would prefer if you didn't hold on to this."
%  \end{quote}
``people can still take screenshots... But it does, make me feel a little bit more comfortable...'' (P18).
%, but at the same time I'm very aware that people could be screenshotting my content.
% Similarly P17, echoed that
% P4 and P17 shared that they used expiring messages only when sharing intimate content in countries where LGBTQIA+ individuals have fewer rights. 
% P17 commented that because homosexuality was criminalized in a country he was visiting, there were different norms around using expiring messages, 
% ``I only use the send once function in that country I mentioned where it was kind of socially normally. Got a few comments being like, dude, you can't send your picture on and not have once. So I at least like okay, better do it just to kind of go by the norms..." 
% Despite being skeptical of the feature and commenting that it, "is a little bit stupid because if you take a screenshot, the other person won't know it", P4 still mentioned that, "when I go to Morocco, which is a more dangerous place for homosexuals, I use this expiring pic feature."
%  expiring messages are messages that are removed from a sender and recipient's chat history after a certain time period that is either predetermined or based on a timer selected by a sender, depending on the platform. 
%  Participants had used this feature on Instagram, Grindr, Snapchat, and WhatsApp. 
%  P4, P5, P14, P23, and P24 described using it with strangers or recipients that they had less established trust with. 
% expiring messages were also used to calibrate the sensitivity of an image, "if the image disappears, I can be more explicit. However if the image is kept in the chat, I make it less explicit" (P14). 
%  For instance, P14 shared that, 
%  ``if I don’t really trust the person I choose the option in which you can display the photo just for once [...] if the image disappears, I can be more explicit. However if the image is kept in the chat, I make it less explicit." 
 
%  P19 also added that although they had not used expiring messages, they would find it useful if they were to share intimate content with a stranger.
 % if it's someone I recently met I always prefer the autodeleting option
% if it's someone Im in a relationship with, I even like that they store my content (P24, Pos. 274-276)
 % Yes, yes, but I haven't used it. I think it would be good for a casual sending with a stranger. (P19, Pos. 288)
% Although a third of sex working participants used expiring messages, many did not.
% such as P46  who used the feature to provide variation in how they advertise or distribute images to clients, many sex workers did not. 
% Aside from security concerns, a few sex workers feared that expiring messages would jeopardize trust with clients. 
% %  were also surfaced such as sex-work specific ones that included the potential for clients 
% to feel that they had been scammed (P9), the possibility of jeopardizing trust with a client (P44), and lower pricing for disappearing images (P49).
% I think a lot of clients also will be afraid that we scammed them. This has happened lately a lot.  (P9, Pos. 180)
  % Oh, yes. Mainly for fun. Like, I think this is like, it gives kind of variation in terms of how the images can be distributed, which is nice for... in terms of like advertising and being able to send like teasers and stuff like that. (P46, Pos. 222)
% I think that the system for sending expiring pictures on WhatsApp is a little bit stupid because if you take a screenshot, the other person won't know it. I really don't understand why some people keep doing it like anyway. Because it doesn't guarantee safety at all. But otherwise, I've been coming across. No, not really. (P4, Pos. 249)
% This feature proposed by Grindr of sending expiring expiring pic pictures, prevents people from taking screenshots and whenever they use the screen recorder to get to, to either, I forget the word, whenever they use the screen recorder the video appears completely black, so it's very convenient. So yeah, when I go to Morocco, which is a more dangerous place for homosexuals, I use this expiring pic figure. (P4, Pos. 201)
Those who did not use the feature had security concerns. They wanted to retain documentation of interactions with recipients in case of future harm, or because it
% Among participants who did not use the feature, most did not do so because they felt that the security concerns described above negated the potential protections; because they wanted to retain documentation of their interactions with recipients in case of future harm or because they were concerned that expiring messages ``
% they felt the feature incentivized recipients to store content. Regarding the latter, P31 explained %that  Participants also had the additional concerns that content would still be stored on a platform's servers despite being deleted for recipients and that for recipients they had negative interactions with, the context in the chat history would be lost. P31 added the 
``sort of invite[s] people trying to screenshot...
[because] it almost creates this environment of, oh, this is secret, which sort of invites people to be like, Oh, I'm going to try and hold on to it'' (P31). Relatedly, sex working participants feared that using the feature would jeopardize the perception of trust with clients. 
% \allison{wow fascinating... and this didn't come up with recreational sexters, like it would call trust into question in a romantic relationship?}



%   (P18, Pos. 112)
% I think I think that the view once feature is really good . But that doesn't make it like 100\% secure, you know, someone can screenshot that. Someone could, you know, take a picture with another device. Right?  (P13, Pos. 229)
% Yes, now I try to think if you could also maybe you could also leave it without deleting it automatically. Now that I'm thinking of it but then it were like if you had to if you wanted to delete it automatically it had like a small period of time. I think that was my complaint from the time I was using it. (P15, Pos. 245)
% AGAINST:
% P41, P43, and P50 also shared these same concerns but unlike the previous participants mentioned, these concerns deterred them from finding expiring messages useful.
% Participants also had the additional concerns that content
% % P10 added that they were concerned that content 
% would still be stored on a platform's servers despite being deleted for recipients and that for recipients they had negative interactions with, the context in the chat history would be lost. 
% % vital information in the chat history would be lost. 
% % Aside from security concerns, a few sex workers feared that expiring messages would jeopardize trust with clients. 
% % %  were also surfaced such as sex-work specific ones that included the potential for clients 
% % % to feel that they had been scammed (P9), the possibility of jeopardizing trust with a client (P44), and lower pricing for disappearing images (P49).
% % % I think a lot of clients also will be afraid that we scammed them. This has happened lately a lot.  (P9, Pos. 180)
% % Well, maybe for other people, not for clients, because the things that I, you know, send them this, so they feel trustworthy to me. So this is good for my work, but it's really interesting for any other situation. I don't know, like more in personal life or something. P44
%  % I sell pictures that... I don't know how low it could be priced for pictures that disappears. (P49, Pos. 260)
% % P37 also added that not only did they not find expiring messages useful, they were concerned that if they had blocked someone or wanted to not interact with them again, they would not have the necessary chat history to remind them of previous interactions. 
% % Similarly, P4, P38, P43, P51 also preferred to have a record of previous conversations to keep track of information someone had share with them, for sentimental reasons, or to view intimate content they had received again.
% % See that, I think it's good. But on some level, does it disappear? To me, I'm like, that sounds like a good idea. But that data exists on my phone and then is sent through servers, so exists on the servers, which will keep a record just because servers can't decide not to, like even if they disappear, they don't necessarily disappear entirely. And you know, there's always a worry for me of like, well, someone could dig it out. If they were determined enough to  (P10, Pos. 355)
%   % I personally don't like it. Not that it's a bad feature. But because I'm forgetful and like, if I were talking with somebody, and they send me a disappearing photo, in the million photos that I've seen in my life, if it's not there next time I open the chat. I'll be like, Oh, but can you send it again? (P51, Pos. 365)
% % Oh, no, I do not like that feature. I honestly, I do not like it, if I trust the person 100\% for me will be the best option is to feel mutual trust, and then keep those photos until we no longer see each other. And then delete them. Because I mean, to be honest, it's a nice feeling to say, hey, (inaudible) somebody if you're into this person. And then you go back and read or see the photos that you exchanged with them. It's a nice feeling. But at the same time, if you do not have that trust, and you don't know that later on, they will delete it. Of course, that's... (P43, Pos. 264)
%  % Meh. I like to have a bit of a record to be fair.  (P38, Pos. 261)
% % Heard of it too, but don't think it's really useful as you can still take screenshot (and I guess there is still other methods to keep messages somewhere) (P41, Pos. 127)
% % I just, I don't really bother with it. I feel like even with disappearing content, they can film it with another camera, or they can take a screenshot of it.  (P50, Pos. 174)
% % With this new features with you know, the image that you can view only once and obviously, that's not the best option, because it turns out that people can just take a screenshot and then you will not even know about it.
%  % (P43, Pos. 108)
%  % um, I do not see how this protects me, actually.  (P37, Pos. 333)
%  % I was a way of if I'm not very careful, someone that has bothered me in the past, but not as much as blocked them will contact me again. And I will not remember that he was an asshole.  (P37, Pos. 337)
% % I think that the system for sending expiring pictures on WhatsApp is a little bit stupid because if you take a screenshot, the other person won't know it. I really don't understand why some people keep doing it like anyway. Because it doesn't guarantee safety at all. But otherwise, I've been coming across. No, not really. (P4, Pos. 249)
% % I will always end up saving some of the messages to to make sure I remember information about the person I'm talking to because I talk to so many people I cannot remember where they all live or what they do for a living or the age or basic information. So I don't really like the the messages can be, can disappear afterwards. But I would like to be able to delete the messages myself afterwards. (P4, Pos. 277)
% Lastly, P31 voiced the concern that expiring messages, "sort of invite people trying to screenshot [...]
% % or like if screenshotting is not possible, other ways of collecting stuff, because it, 
% [because] it almost creates this environment of like, oh, this is secret, which sort of invites people to be like, Oh, with that, I'm going to try and hold on to it."


% Rules
% there was a period where I sort of only was sharing things from neck down. And now that is still more or less the norm. But then if I really trust the person, or as I said, if it's a lover or friend, then I, yeah, if a portion of my face, or if my face is in it, I don't really mind that much. But not to strangers, I think. (P5, Pos. 355)

% Yeah, I suppose. Yeah, that's definitely true. Because there's sort of like a thing for me where.. So I have kind of, like, I guess, hierarchies of how much I trust a person, right? So if I'm, like, initially, sort of like seeing someone and I'm like, I don't know, like, maybe they could do something nefarious with this, I'll never show them and send them anything that involves my head. Right? So I don't necessarily care if it's like not the most encrypted messenger in the world, if my head is not involved, right? I'm just like, well, whatever. Like, you can't necessarily identify me or whatever. So with that, and then if it's, you know, someone that I have, like a relationship with, and I kind of trust them a bit more than it's like, well, if somebody hacks this, that's kind of, I guess, I kind of see the moral thing on them. I'm like, Well, if that leaked, leaked out to the general public, you know, I'm lucky enough that I wouldn't, I would just be like, Oh, well, you you're the one who did something wrong there. And because of how my life is, that wouldn't, it wouldn't like bring me down or something like that, you know?  (P12, Pos. 37)
% So most of the people that who have like things where I am identifiable, those are people that I really trust, you know, so, and I don't even if I've stopped dating them or something like that, I don't think just because of who they are. That's that's the sort of thing that they would do. Yeah. P12

% also, only on DM I send my face. P49

% POST HARM
% But I do remember that future photos was... were really less revealing than they used to, and it was definitely low revealed... you cannot recognise me on the photos later on. (P43, Pos. 52)
% Okay, yeah, I mean, your background, maybe you need to hide your backgrounds a little bit. And even if the background is identifiable, and your face is not identifiable, it still makes the case like, okay, a really big difference. So I think the most important thing is that your face is not in it. (P43, Pos. 216)

% It's usually like for... with my like, old customer base it's usually with my face and everything. But... and it also comes to like, the rate for certain... it's more expensive to like, get my face. And also for the videos, it's like, kind of premium content. But with the newer base, I prefer under the images, I prefer to keep my face off of it. Yeah. (P1, Pos. 212)


% 52: in the pawst only no face


% Encrypted folders (what does this mean?) (P8)




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% PASSWORD SAFETY %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Password Safety}


%\elissa{i would separate picking an app b/c it offers password protection vs. general password safety which we need to move to safety maze - security (7.1) }
%\sharon{what about setting a password? also kind of safety behavior (i.e., safety maze)?}

% notes-- themes: 
%% using password for phone but not apps within phone (WhatsApp. photos app) - P21 P26 P44 
%% password for folders - P8 P47
%% strong or different passwords or 2FA - P33 P7 P12 P29 P28 P42
%% biometrics - P13 P1 P29

% % storage: % 
% Password safety refers to both the user's decision to implement password protection and a platform's built-in ability to set a password. The majority of users referenced setting password protection on their phone, laptop, or hard drive (i.e., personal devices), although some users also mentioned Google Drive (P12, P42) or Tumblr previously (P39). P8 and P47 opted to set additional passwords on folders within their personal devices. Participants ranged in their adherence to strong password security measures. Some participants (P7, P12, P28, P29, P33, P42) explicitly mentioned setting strong passwords, implementing two-factor authentication, or utilizing a password manager and others (P13, P29, P1) said they employed biometric measures (e.g., FaceID or TouchID) to increase their security (P13, P29, P1). On the other hand, some users admitted being more lax about password safety overall. For example, P50 mentioned "Yeah, I try to use a password. I'm also not so good with that. I sometimes take it off my phone, and then I forget to put it back on. Yeah, so I'm aware that I could do more, but sometimes it just slips a bit." Other participants (P47, P49) echoed these sentiments, noting inconsistent password safety behaviors. (\todo{password sharing/device sharing})

% We found that the majority of participants mentioned password safety at least once and most implemented passwords to reduce the risks of hacking or theft. Other participants utilized password protection to prevent unintentional viewing \sharon{word choice?}, such as device sharing or shoulder surfing. For instance, P48 mentioned password protecting folders: "At the time, [my children] didn't have their own devices so they would sometimes use mine to play a game or do a little search. I knew they wouldn't look for things, but it made me uncomfortable knowing they could find content by accident, so [password protecting folders was an] extra precaution."

% % sharing:
% Some participants were also mindful of their recipients' password security. P22 said, "I always ask if they have passlock in their phones" before sending intimate content.

% %Participants often selected sharing or storing methods based on the ability to set a password.  -- TO DO: FIND P#s

% When participants were asked about their ideal design, many (P11, P12, P19, P27, P51) explicitly mentioned password protection as an integrated feature. 

\smallskip
\noindent\textbf{Screenshot Notifications.}
%\lucy{@sharon}
%%%%%
% \lucy{TODO: count on how many used and mainly for what}
% Screenshot notifications alert senders of
% when recipients take screenshots of content.
A third of participants used screenshot notifications. This was more common among recreational participants
% it was mainly within the context of a specific app known for the feature and 
% many wished for wider adoption. 
% Screenshot notifications were more commonly mentioned among recreational participants
who primarily used them to calibrate trust and 
% The vast majority of users (count: 42) found the feature useful and one-fifth of participants were more likely to use a platform that included screenshot notifications. 
% P2 commented, "
% I think it's better to let people know when an image of theirs has been stored, especially if it's like a expiring message because 
% it empowers [people] to make decisions about whether to continue sharing messages."
``make the confrontations and the discussions that you need to do to be safe'' (P10). 
% Additionally, P5 shared that in one instance, they asked a recipient to delete an image after receiving a screenshot notification. 
Even though many found the feature to be useful, they were aware that the notifications could be bypassed (e.g. capturing with another device).
% ``There's always people who can figure out ways around it, like taking a picture of another screen with another phone" (P31).
% While most participants found the feature useful, 
% There was a subset of participants that did not find the feature useful or necessary
% % For example, P3 said, "If people want to download my images, they can just click the button, click download, I don't really care. I don't really mind. They're free to do it." P7, P19, and P26 also expressed similar sentiments, and P44 noted that
% such as P44, 
% "I can see how it can be useful for a lot of sex workers. [...] But for me, I don't know, maybe the thing for the screenshots, but actually, I don't care."
% They added that it did not offer sufficient protection since it fails to prevent
% Finally, a number of our participants expressed a desire for full prevention. They noted that a notification might be helpful, but it fails to prevent 
% the recipient from taking a screenshot or recording in the first place. P4 mentioned that they only used a method that contained more robust screenshot prevention,
% \begin{quote}
    % "So Grindr enables you to create an album where you can store photos. And it enables you to give access to this album, so to give access to all of the pictures that are inside of the album at the same time, and 
    % I find out that it's impossible, no, probably not impossible, but it's pretty hard to take screenshots of the pictures [while using this app]. 
    % that are stored in this album. [...]
    % And so this method became the best method to guarantee discretion and security among all the platforms where you can share this kind of pictures, because you can take screenshots of Snapchat, of WhatsApp, of Instagram. And sometimes it notifies the person you're talking to. But there's only on Grindr that you cannot, like the application itself prevents you from taking screenshots, which is great. 
    % With people I don't know, and people I'm absolutely not, I have no trust in, I only send pictures through the album of Grindr."
% \end{quote}
% \lucy{Move this paragraph to safer futures?}

% Themes:
%% empowering/informative - P2 P10
%% more likely to use platform w this feature/dream design - P2 P8 P12 P18 P21 P22 P30 P35 P37 P43 P46 
%% don't care - P3 P7 P19 P26 SW44
%% prefer prevention entirely - P4* P13 P15 P16 P18 P40 P55
%% also want screen recording notification - P11
%% notification doesn't do anything - P4 P35 P32
%% ways around it - P11 P17 P24 P26 P28 P31 P34 P35 P50
%% useful - P5 P8 P9 P10 P11 P11 P12 P14 P17 P52

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% PRIVACY SETTINGS %%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Privacy Settings}
% %\lucy
% \lucy{More quotes in comments---will condense section into a sentence}

% %P42 ``I think the good part of Google Drive is that you can do very specific... like content protected with passwords that you can sell the password to access, things like that. To make it easy and more or less secure to...''

% P19 ``the good thing with telegram is that if you send or receive photos, you can like select, you can choose if you want the photos to be shown on your photo gallery. So I usually deselect that. So I am aware that my photos won't be in my photo gallery and only will be in the app.''

% P10 ``so you can you can like censor images on Discord like you can so it, you have to press the spoil button.''

% %P17 ``And WhatsApp, I have my own folder where I keep them, which is kind of separate from the other folders, again, to stop the scrolling issues when you're looking for a folder amongst your friends and one pops up.''

% %P17 `` Grindr increased its functionality. If you could upload stuff to Grindr specifically include like a phone. And that was kind of the main one essentially. So you keep all my nudes there and delete them everywhere else.''

% %P13 `` So I use, like Google Photos. So I guess that's cloud and an app. Yeah. And they have like, a locked folder within that.''

% - Secret Conversation in Facebook Messenger 

% - that Kik is not connected to a phone number 

% - being able to turn off Auto-download (I think whatsapp or telegram) 

% - Grindr consent to receive profile status


% - "in Telegram, for example, you can delete everything for yourself and the other person and erase it from it's not stored anywhere, it's not backed up or anything," P35


%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% E2EE %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\smallskip
\noindent\textbf{End-to-End Encryption.}
End-to-end encryption (E2EE) ensures that only a sender and their intended recipient(s) can view a message.
% , preventing a third-party, such as a messaging platform, from viewing it.
Once an E2EE message has been delivered, it carries similar risks to unencrypted messages: the recipient can still
store or share it. Over a quarter of participants actively used E2EE or considered it to be useful (excluding those who happened to use platforms with E2EE but did not mention it). For a few, E2EE alleviated their concerns about unwanted access by a platform or government entity: %P47 who says that E2EE "addresses my own actual concern, which is exposure, not by an individual, but by a platform or like an infrastructure itself". 
% P26 added that they used end-to-end encryption to defend against theft, which they felt was less within thei
% \begin{quote}
%\lucy{Alt quote: 
``There are basically two possible attackers. Like either the person I'm sending this to or someone from the outside trying to break into systems and stealing data. [...]
% Since I want the recipient of the message to see the picture and therefore be able to leak them anyways, it's just not an attack I care about. So I leave the security there. 
I mostly care about someone from the outside able to steal pictures'' (P26). 
% And as I said, for me that scenario, like the risk that this... of this actually happening is acceptable, but in 
% \end{quote}
P10 added that they valued E2EE because, ``if there's anything I don't want, it's the government knowing details of my personal life and seeing my tits.''
% Others found E2EE improved their trust in that platform (see Section~\ref{subsect:decisions-safety})  even if it did not protect against any IBSA-specific threats they anticipated: ``
% ``I think because [E2EE is] the most standard thing for texting now...
``It [is] suspicious if one app doesn't have [E2EE]'' (P15).
% "they use end to end encryption, which gives me more trust. (P13, Pos. 181)"
On the other hand, a sixth of participants did not trust E2EE, believing that it did not work or could be broken by a platform or police if needed. ``If someone wants the data, they will get their hands on it anyway. And if that someone is the police, they will just force companies to give that to them. No matter how well encrypted it is'' (P50).
% Others did in fact use the availability of end-to-end encryption as one of the factors in choosing a platform to send and receive intimate imagery. 
% No, I mean, Messenger I have been using for texting, but the secret conversation like extension only for that. (P15, Pos. 49)
% \lucy{had observation and wanted to note somewhere that E2EE as a feature might not be super useful in this context but it maybe provides trust that the platform takes privacy more seriously such as in commented out quote below}
% they kind of say, often that they use end to end encryption, which gives me more trust. But, yeah. Yeah, I don't really know how to answer that. I guess we just haven't. I just have moved away from those other apps towards WhatsApp as the main messaging one. (P13)



\smallskip
\noindent\textbf{Watermarking.}
% Use P: 5, 17, 27, 31. 33, 34, 35, 37, 40, 48, 50, 52, 53 (13)
Watermarking, which is used to apply a visible or invisible signature to content, was mainly used by the sex workers we interviewed. Overall, a quarter of participants used watermarking for four reasons. 
First, to deter others from stealing and re-selling content:
%\begin{quote}
     ``If your content's watermarked, then other platforms won't allow it to be uploaded'' (P35). % And I think that's the thing we have this conversation with these collect collectives of sex workers where they just like watermark your images, watermark your images, because it provides a lot of protection. And like,
    % "If you brand yourself in a specific way, 
   % "...it highlights the fact that this is a service, and you have control over this service. And then other platforms where if it does get leaked, or if boundaries are crossed, these platforms won't accept it if it's been watermarked as something else, because they then know that it's not." (P35)
    % , unless you don't have proof that this has come from that person that's been watermarked, then it won't be posted. So that's kind of reassuring, but again, can still there's still ways around that if people really want to ruin your life. Sorry, I'm being really dramatic. (P35, Pos. 237)
%\end{quote}
Second, to proactively prepare for future removal of nonconsensually shared content since ``when you report on social platforms, you have proof of ownership'' (P1). P18, however, surfaced the concern that its use could reveal one's identity and 
% potentially putting you at even more risk because you're trying to have this thing taken down. [...]
% So I think it would be really important for companies to really think about how they are going to deal with people's requests to have material taken down and what they can do to protect people. 
% And yeah, it would be nice to have things watermarked, but 
``that could also be used against people like, oh, it's the same girl in all these photos, collect them and put them in a folder together.'' 
Third, to subtly imply that an image should be kept private. P31 started writing a sentence onto an image to let recipients know that it is only intended for them as a ``way of trying to...put the accountability on the person who is sharing it instead of me.'' 
% So like, recently, a little bit more, I've put like, texts in the images themselves. So like, when I edit them,
% I'll put like, a little sentence in the image not to like hide anything or to, I don't know, watermark anything, but just to sort of be like if someone would receive that they would know who it had originally been sent to. 
% And like that it was meant for only them and so obviously, they can then see that that person has crossed a boundary. So I hope that sort of deters people from sending them on. (P31, Pos. 157)
% it shows that it's yours. And like in that way, it can become a bit of an advertisement or something. But in personal life, I think also the way I do it, it just like I think it is my way of trying to implement sort of the like, putting the accountability on the person who is sharing it instead of me. Like who's non consensually sharing it instead of me sending it so like by including their name in the image, you sort of implicate them into it more. (P31)
Or, fourth, because it was applied automatically.  P5 explained that on a dating app, 
% ``When you...look at someone's picture full screen, 
``It always displays the username [on the content]...
% Everyone has this...six, seven digit user name...
[displaying] it deters people from pretending to be the person in the photo or spreading your photo as theirs.''
As with other strategies, the usage of watermarks was caveated by acknowledgements that they could be removed or altered.


\smallskip
\noindent\textbf{Retroactive Unsend.}
Around a quarter of participants manually deleted intimate content from messaging  histories such as through using an ``unsend'' feature to prevent a recipient from storing their images.
% after that, I just delete them for myself. And, of course, I we are in communication with a partner to do the same (R8, Pos. 25)
% another practice mentioned was deleting intimate content from text exchanges (P4, P5, R8, P11, P17, P18, P19, P21?, P22?, P30, P34, P45, P32).
% On some platforms, such as Grindr or WhatsApp, users are given the ability to delete the image from both their own view of the messaging history and their recipients', which participants utilized. 
P32 described waiting for a client to view an image. After they receive a read receipt, they delete the image from their 
% WhatsApp 
conversation history. P5 added that, ``So sometimes if I feel like you know, a person's acting fishy, then I either delete the messages or delete the photos.''
% If it's photos that I feel uncomfortable with, like on a personal level, usually, it's like in the moment of arousal and you're sexting, then I feel comfortable sending these, especially 
% "...I have a few guys that I'm seeing that specifically request these and it makes me really happy to provide them with this material. But then afterwards, after I've sent them, I usually delete them."
% P30, commented that, "I used to delete them in the in the conversations like in the WhatsApp messages where I send them but I don't delete them. Because it was more traceable this way. And I didn't like them in the conversation." 
% Yeah, I mean, as soon as... my own ones I delete as soon as I've kind of sent them unless it's the ones I kind of send regularly if that makes sense. Other people's, I think get deleted automatically off Grindr. Unless it's sent to me on WhatsApp, in which case, I'm not sure if they are deleted unless they come up when I'm scrolling and I delete them then, essentially. But how often I delete them, it depends if they're ones I know I don't... I wouldn't want to look at in the future then they're kind of gone. And the old ones are gone, too. I suppose. So, I mean, I suppose pretty much weekly when I was on Grindr, I probably would have went through and chose the ones I didn't want. (P17, Pos. 33)

% So sometimes if I feel like you know, a person's acting fishy, then I either delete the messages or delete the photos. Or sometimes I block them because that sort of also keeps them from seeing the photos. (P5, Pos. 217)
% Oh, yeah. I think I only do share when my boyfriend shares first, that's for sure. And I don't send this... I don't share disappearing, no, but I do delete everything in my conversation afterwards. (P45, Pos. 213)
% No, I don't think so. I just, you know, maybe the only thing that I do is like, I never like send the photos and you know, put my phone away for a while. I always wait for the client to see the photo. And when I see the you know, the sign message that it was seen I delete that, so I can be sure that he saw the picture, but it's not on the internet anymore. Of course, that's not... everything that is on the internet stays in the internet. But anyway, I feel more comfortable when I delete the photo. (P32, Pos. 120)

%%%%%%%%%%%%%%%%%%%%
% METADATA REMOVAL %
%%%%%%%%%%%%%%%%%%%%

\smallskip
\noindent\textbf{Storage Strategies.}
To defend against storage-related threats on their own devices (e.g., hacking, unintentional discovery, device theft), around half of our participants proactively deleted their own stored content:
``my [\textit{cloud storage}] will send me like, memories of [intimate content]... coming up on the screen [when] I'm just like, trying to sip my tea and have a relaxing day. That's where I'll be like, yeah, get out of here" (P46).
A quarter were mindful about their authentication practices---choosing to use strong passwords, 2FA, biometric authentication, or password managers. Finally, a quarter of participants chose to store content in local storage (or disable automatic backups) while another quarter used a hidden folder, which excludes selected photos from a user's photo gallery and places them into a designated folder (e.g., Apple \cite{apple_hide_nodate}, Samsung\cite{samsung_what_nodate})
to prevent unintentional discovery.
% of intimate content.
% ``if I have a lot of sexy pictures kind of in a row in my camera roll, then I will move them into a different folder" (P29).
% ``...sometimes when I'm just going through like, my regular day photos and like nudes will pop up, that doesn't happen anymore" (P46).



%mployed strategies around deleting stored content, hiding it, and/or applying different forms of authentication. This is described in more detail in Appendix \ref{subsect:storage-strategies}.

% `For any intimate photo sharing app, I would hope that that would be in there by default, and it wouldn't be able to be turned off." P2 
%Of the safety strategies they used, a few participants admitted that they were less strict about doing metadata removal and that it is, ``something that I...not only forget, [but] sometimes cannot [be] bothered to do" (P37).
% %\lucy{@sharon}
% % themes:
% %% useful - P2 P3 P4 P6 P7 P9 P10 P12 P13 P14 P15 P16 P18 P21 P22 P23 P24 P26 P27 P29 P30 P31 P33 P35 P36 P38 P40 P41 P43 P44 P46 P47 P50 P52 P1 P55 P20
% %% not useful - P8 P19 P28 P48 P51
% %% would not use app without/more likely to use app with - P2 P12 P26 P46
% %% in theory but not practice - P5 P11 P27 P31 P37 P39 P42 P49
% %% should be there automatically/by default - P2 P6 P25 P33
% %% in control/security - P9 P14 P34
% %% no metadata in the first place - P15 P23 P33
% %% only useful on public data - P26
% %% not enough - P41 P47 
% Metadata removal eliminates information about an image, such as GPS location, owner name, date/time of creation, etc.  \lucy{Todo count on how many ppl use it and in what contexts}
% \lucy{Who normally uses and how?}
% % With the exception of five, participants largely found metadata removal to be a useful feature.
% In fact, P2, P12, P26, and P46 were more likely to use a platform with metadata removal. P2 mentioned, "I think it would be a big negative if that turned out to not be done automatically. [... ] But I would think for any intimate photo sharing app, I would hope that that would be in there by default, and it wouldn't be able to be turned off." Other participants (P6, P25, P33) shared a similar desire for metadata removal to be integrated into a platform by default. P9, P14, and P34 felt they would be more in control of their data and security if they were able to remove metadata from their content. 

% Some participants (P5, P11, P27, P31, P37, P39, P42, P49) described metadata removal as useful in theory, however they themselves did not consistently utilize this feature. P31 shared, 
% \begin{quote}
%     "[It's] something I think about very often, but never actually do. [...] especially when it comes more to things like sex work, risks of doxxing and those kinds of things. It's just really helpful to have that removed. And I don't think we're all thinking about it all the time. And you kind of forget it, because it's not, it's not right there on the image, you don't see it directly, you need to like go out of your way to find it."
% \end{quote}

% A few participants (P15, P23, P33) expressed a desire for the elimination of metadata entirely. P15 said, "I mean, ideally, I wouldn't like [metadata] to be stored in the first place. But if it had to be stored then yeah, like, I think the metadata removal would be better from now." Additionally, P41 and P47 both thought that metadata removal was not sufficient to truly protect users: "I think it's useful in a way for privacy but not perfect" (P41).










\subsection{Learning}


\smallskip
\noindent\textbf{Behavior Change.} 
%\lucy{@Elissa this section feels out of place here but not sure where else to put it. Also need to edit text to cut down---Hmmm ok after reading thru this again, I feel like the most interesting part maybe is about how behaviors change with age and maybe we can cut the other stuff. I think a noticeable amount of participants emphasized how they were more careless when they were young. Maybe this could turn into a recommendation about harm reduction and education or we not touch it...}
\label{subsect:behavior-change}
%% themes:
% trust/boundaries/consent - P21 P29 P30 P45 P52
% changes in technology - P2 P6 P12 P29 P43 P46 P47 
% for safety/security - P8 P29 P33 P34 P42 P43 P49 P55
% with age/experience - P2 P5 P6 P7 P12 P14 P18 P23 P24 P29 P31 P42 P46 P49 P50 P51 P52 P32 P20
% political landscape - P4
% proliferation of sex work platforms (e.g., only fans) - P4 P41
% acceptability/reduced stigma of sending nudes - P6 P14* P32
% empowerment - P38
% because of IIA - P21* P35 P38 P43 P45 P50 P20
% pandemic - P27 P38
% platform reputation - P37 P55
% $$ - P38 P41
Participants did not use the strategies summarized statically. Many changed their behavior over time for a number of reasons, the most common of which was getting older and gaining more experience: ``When I was a bit younger, I would not be so discerning with who I would share stuff with... But now I am much more kind of strict'' (P29).
% , I suppose, with people who I send things to" (P29). 
About a third of participants echoed these sentiments but another third became less concerned: ``over time you grow up, you mature...
% sexually and in many other ways... 
I know better what I need'' (P51).
% and understand that the internet is a vast, vast, vast, vast space."
% P32 commented that in their personal life, ``I feel more like chilled and comfortable when I do the private, nude pictures."

 % P51 commented that they were less afraid , 
% `before, I think I was a lot more cautious. But I think ``after like quite some years of doing this, and never having had a problem, I'm kind of like much more settled about it."
% ``over time you grow up, you mature sexually and in many other ways... I know better what I need and understand that the internet is a vast, vast, vast, vast space."
Other participants naturally adapted their behavior as technology changed such as transitioning from email to modern platforms. 
% ``I started using actual platforms to send them rather than uploading them somewhere, on my email because that was more common back in the day...'' (P47).
% I now use the built in features of the app'' (P47). 
Sex workers also mentioned changing which platforms they used: ``Yes, when I started I was selling pictures only [directly] because I was also working [offline], [now] I've tried platforms like [\textit{adult content platform}]'' (P41).% Other sex workers mentioned changing platforms due to the COVID-19 pandemic forcing them to find virtual work "At the beginning of the pandemic, when we like had to switch from full service, because I didn't really do much virtual before the pandemic, I was actually very hesitant. But as I say I had to fucking survive, so I had to do, and even to this day, like, I keep playing with the idea 'Okay, I'll go on Chaturbate.'"

Finally, some participants made explicit changes to their behavior for safety or security reasons. Some chose to do so as they gained more knowledge or expertise around safety practices. For example, P34 mentioned ``I was showing my face and sharing personal details at the beginning. I don't do that anymore. Because I don't know anything about clients.'' A sixth of participants, both commercial and recreational, shared similar sentiments. 
% when I got older. And when I was almost graduated from high school, I was thinking, `no, I shouldn't do that anymore.'"


%\lucy{@Sharon seems like there's something missing here!}
%\elissa{+1 feels like being victimized would be a source of behavior change we should definitely mention!}


